Myopic Bayesian Design of Experiments via Posterior Sampling and Probabilistic Programming

We design a new myopic strategy for a wide class of sequential design of experiment (DOE) problems, where the goal is to collect data in order to to fulfil a certain problem specific goal. Our approach, Myopic Posterior Sampling (MPS), is inspired by the classical posterior (Thompson) sampling algorithm for multi-armed bandits and leverages the flexibility of probabilistic programming and approximate Bayesian inference to address a broad set of problems. Empirically, this general-purpose strategy is competitive with more specialised methods in a wide array of DOE tasks, and more importantly, enables addressing complex DOE goals where no existing method seems applicable. On the theoretical side, we leverage ideas from adaptive submodularity and reinforcement learning to derive conditions under which MPS achieves sublinear regret against natural benchmark policies.

==> archive/intro_may20.tex <==

\section{Introduction}
\label{sec:intro}

%To mention,
%\begin{enumerate}
%\item differentiate between OL, RL, submodularity settings
%\item why  myopic strategies
%\end{enumerate}

%% Related work
%% \begin{enumerate}
%% \item Connectio
%% \end{enumerate}

%To cite:
%~\citet{chen2017near,gabillon2013adaptive,gabillon2014large}

%\towillie{In addition to the stuff that we discussed today,
%\begin{enumerate}
%\item How PP enables us to do this.
%\item How many problems in science and industry have very specific objectives:
%not just vanilla AL or BO.
%Hence, we need a flexible framework to do this.
%\item Why we need to incorporate domain expertise in the form of a prior.
%\end{enumerate}
%}

Many real world problems fall into the design of
experiments (DOE) framework, where one wishes to design a sequence of
experiments and collect data so as to achieve a desired goal.
% Many industrial and scientific problems can be treated in the 
% design of experiments (DOE) framework, where the goal is to design a sequence of
% experiments and collect data so as to achieve a desired goal.
% so as to minimise a given penalty $\penl$.
% In many practical problems of interest $\penl$
For example, in electrolyte design for batteries, a chemist would like
to conduct experiments to measure the battery conductivity
in order to identify an electrolyte that maximises the conductivity.
On a different day,
she would like to conduct experiments with different electrolyte designs to
learn how the viscosity of
the electrolyte changes with design.
These two tasks,
black-box optimisation and active learning, fall under the umbrella of
DOE and are pervasive in industrial and scientific applications.

% along others fall under
% the umbrella of DOE,

% are pervasive in industrial and
% scientific problems

% Some common examples are optimisation and active learning.
% In the former, each experiment can be interpreted as an evaluation of some black-box
% function $f$ and the goal is to find a design that maximises $f$.
% For example, in electrolyte design for batteries, a chemist wishes to identify
% an electrolyte that maximises the conductivity.
% In active learning, an experiment at  $X$ can be interpreted as a draw from the
% discriminative distribution $\YX|X,\theta$; our goal is to obtain data in the form
% of $(X,\YX)$ pairs and estimate the parameter $\theta$ from this data.
% For instance, the above battery chemist may wish to conduct experiments at
% different electrolyte designs, in order to quickly learn how the viscosity of
% the electrolyte changes with the design.

While several methods exist for specific DOE settings, real world
problems are broad and complex, and specialised approaches have
limited applicability. Continuing with the electrolyte design example,
the chemist can typically measure both conductivity and viscosity with
a single experiment~\citep{gering2006prediction}.
Since such experiments are expensive, it is 
wasteful to first perform  a set of experiments to optimise conductivity 
and then a fresh set to learn about viscosity. 
It is preferable to design a single sequence of experiments
that simultaneously achieves both goals.
In metallurgy, one may wish to conduct experiments
to identify phase transitions in an alloy as the composition of metals
change~\citep{bunn2016semi}.
Here, and
elsewhere, both the model and the goal of the experimenter are very
application specific and cannot be simply shoe-horned into
formulations like black-box optimisation or active learning.


% While there are several methods for specific applications such as the above,
% real world DOE tasks are more broad and complex.
% For example, in the above electrolyte design setting, we might be able to measure
% both the conductivity and viscosity via a single experiment~\citep{gering2006prediction}.
% Since each experiment is expensive, it is inefficient to first
% perform a set of experiments to optimise conductivity and then a second
% set to learn viscosity.
% Rather, the chemist prefers to design a single sequence of experiments
% that simultaneously achieves both
% objectives.
% Similarly, in metallurgy~\citep{bunn2016semi}, one wishes to conduct experiments
% to identify the phase transitions in the alloy as the composition of different metals
% change.
% The goal in these and similar tasks are very application
% specific and cannot be simply shoe-horned
% into broad categories such as optimisation or active learning.
To address these varied applications, we develop a
general and flexible framework for DOE, where a practitioner may
incorporate domain expertise about the system via a Bayesian model and
specify her desired goal via a penalty function $\penl$, which can
depend on unknown system characteristics and the data collected during the
DOE process. We then develop a myopic strategy for DOE, inspired by
classical posterior (Thompson) sampling for multi-armed
bandits~\cite{thompson33sampling}. 
% 
Our approach has two key advantages. First, the Bayesian formulation
allows us to exploit advances in probabilistic
%programming~\citep{neiswanger2015embarrassingly,tran2017edward} to
programming~\citep{carpenter2017stan,tran2017edward} to
incorporate domain expertise without introducing complexity. Since
experiments are typically extremely expensive in applications,
incorporating domain
expertise is essential to achieving the desired goal in few experiments.
Probabilisitic programming offers an elegant method to do so.
Second, our myopic/greedy strategy is simple and
computationally attractive in comparison with policies that engage in
long-term planning.  Nevertheless, borrowing ideas from submodular
optimisation and reinforcement learning,
we derive natural conditions under which our myopic
policy is competitive with the globally optimal one.
Our specific contributions are: % n this work are as follows.
\vspace{-0.03in}
\begin{enumerate}[leftmargin=0.2in]
\item We propose a flexible framework for DOE that allows a practitioner to
  describe their system (via a probabilistic model) and specify their
  goal (via a penalty function).
% state their desired goal in the form of a penalty function.
We also derive an algorithm, Myopic Posterior Sampling (\mps), for this setting.
\vspace{-0.03in}
% which is inspired by posterior sampling.
\item 
We implement \mpss using probabilistic programming and
demonstrate that it performs favourably in varied suite of synthetic and real
world DOE problems.
Despite our general formulation, \mpss is competitive with specialised methods designed for particular problems.
% being a generic framework,
% it performs favourably with methods specifically designed for certain problems.
\vspace{-0.03in}
% \item In our theoretical analysis, we study conditions under which a myopic policy
% may achieve reasonable performance when it does not know or observe the
%  penalty.
% \mpss can be competitive with myopic and globally optimal strategies
% which know the penalty under suitable assumptions.
\item In our theoretical analysis, we explore conditions under which
  \mps, which learns about the system over time, is competitive with
  myopic and globally optimal strategies that have full knowledge of
  the system.
% a myopic policy
% which does not know or observe the penalty, such as \mps,
% may be competitive with myopic and globally optimal strategies
% which know the penalty.
\end{enumerate}

%  Note that the DOE problem is more
% challenging than



% % In this work, we aim to develop a general and flexible framework for DOE,
% % where a practitioner may specify their desired goal in the form of a
% % penalty function $\penl$ which depends on the data collected in the DOE process.
% % Typically,
% % $\penl$ may also depend on unknown problem quantities and cannot be computed from
% % the data alone.

% In this work, we develop a myopic strategy for DOE that is inspired by
% the classical posterior (Thompson) sampling procedure for multi-armed
% bandits~\cite{thompson33sampling}.
% We focus on myopic (greedy) strategies because they are computationally attractive
% than methods which attempt to find the global optimum.
% For example, optimising set functions is known to be a notoriously hard problem.
% However, the seminal work of~\citet{nemhauser1978analysis} demonstrated that
% when the function satisfies a diminishing returns property called submodularity,
% a myopic algorithm which iteratively adds the element that minimises the penalty
% in a greedy fashion can perform competitively with the global optimum.
% A line of work on adaptive submodularity has extended these results to adaptive
% data collection problems~\citep{golovin2011adaptive}.
% However, in these settings,
%  the penalty $\penl$ is assumed to be a function of only the data and hence is known
% to the decision maker.
% In contrast, in this work, $\penl$ might depend on unknown quantities,
% which is considerably more challenging and reflects practical settings for DOE.

% An important practical consideration in many DOE tasks is the incorporation of
% domain expertise.
% One advantage to adopting a Bayesian approach, as we do in this work, is
% that domain expertise can be intuitively incorporated into probabilistic models
% in the form of a prior.
% Moreover, recent advances in probabilistic programming tools and approximate
% inference techniques~\citep{neiswanger2015embarrassingly,tran2017edward} now allows
% practitioners to intuitively specify such domain expertise
%  and perform inference.
% We leverage the advances in these areas to aid in the development of
% an automatic procedure for DOE.
% This allows us to greatly reduce the number of
% experiments that need to be conducted in practice when compared to using
% off the shelf methods.



% \paragraph{Related work.}
% \akshay{This might be better after the setup.}

\textbf{Related work:} The classical results for (sequential) DOE
focus on discrete
settings~\cite{robbins1952some,chernoff1972sequential} or linear
models~\cite{fedorov1972theory}, which enable a more detailed
characterization and refined analysis than we provide. More recent
work in the bandit community studies more complex non-linear
models~\cite{bubeck2012regret,srinivas10gpbandits,streeter2009online},
but ignores temporal dependencies that arise in applications.
% Extending these results, our work
% considers complex models where the agent's decisions affect the future
% state, which is essential in our applications of interest.
% 
We focus on posterior sampling (PS)~\cite{thompson33sampling} as the
bandit algorithm, since it has proven to be quite general and admits a
clean Bayesian analysis~\cite{russo2016information}.  PS has been
studied in a number of bandit
settings~\cite{gopalan2014thompson,kawale2015efficient,kandasamy2017asynchronous},
and some episodic RL
problems~\cite{osband2013more,osband2014near,gopalan2015thompson},
where the agent is allowed to restart. In contrast, here we study PS
on a single long trajectory with no restarts.

Myopic/greedy policies are known to be near-optimal for sequential
decision making problems with \emph{adaptive
  submodularity}~\cite{golovin2011adaptive}, which generalizes
submodularity and formalizes a diminishing returns property.  Adaptive
submodularity has been used for several DOE setups including active
learning~\cite{golovin2010near,chen2013near,chen2017near} and
detection~\cite{chen2014active}, but these papers focus on
characterizing applications that admit near-optimal greedy strategies,
and do not address the question of \emph{learning} such a policy.
% one need not
% learn a near-optimal policy as we consider here.
% For sequential decision making problems with partial observability,
% which we are considering here, adaptive submodularity is a structural
% condition---generalizing submodularity and formalizing diminishing
% returns---under which greedy adaptive policies are known to be near
% optimal. 
As such, these results are complementary to ours: adaptive
submodularity controls the approximation error (the difference between
myopic- and globally-optimal strategies, both of which know the
penalty $\penl$), while we control the estimation error (how close our
learned policy is to the myopic optimal policy that knows $\penl$).
As we show in Theorem~\ref{thm:submodthm}, with adaptive
submodularity, \mpss can also compete with the globally optimal
non-myopic policy.  Prior results for learning in (adaptive)
submodular environments are episodic and allow
restarts~\cite{gabillon2013adaptive,gabillon2014large}, which is
unnatural in the DOE setup.

% Since we are focusing on myopic/greedy strategies, a natural point of
% comparison is the literature on (adaptive) submodular
% optimization. 

% Similarly, most results for learning submodular functions are episodic. 

% The classical results focus on computational issues;
% efficiently optimizing a known submodular function via greedy methods,
% but recent work has addressed various learning problems where the
% function is unknown, as we do here. On the other hand, the results for
% learning submodular functions are episodic, while we focus on learning
% from a single long trajectory (which necessarily requires further
% structure). \akshay{On the other hand, we are not aware of any
%   ``bayesian'' methods for bandit submodular optimization, which we
%   provide here for the first time.}

Our formulation can also be cast as reinforcement learning since at
each round the agent makes a decision (what experiment to perform)
with the goal of minimizing a long-term cost (the penalty
function).
 One goal of our work is to understand when myopic
``bandit-like" strategies perform well in reinforcement learning
environments with long-term temporal dependencies. 
There are two main differences with prior
work~\citep{kearns2002near,strehl2009reinforcement,jaksch2010near,osband2013more,osband2014near}:
first, we make no explicit assumptions about the complexity of the
state and action space, instead placing assumptions on the penalty (reward)
structure and optimal policy, which is a better fit for our
applications. More importantly, in our setup, the true penalty is never
revealed to the agent, and instead it receives side-observations that
provide information about an underlying parameter governing the
environment. Lastly, our focus is on understanding when myopic
strategies have reasonable performance rather than on achieving global
optimality; it may be possible and interesting to extend these results
to the general RL setting.

%  Instead the agent receives
% side-observations that provide information about an underlying
% parameter governing the reward

% However, our the experimental
% design problem calls for 

% several differences to existing theoretical works in RL


% \toakshay{Can you write the Related Work section, and .
% \begin{enumerate}
% \item Compare our results and setting with submodularity, RL, OL etc.
% e.g. reward not observed.
% \item Why people study myopic strategies: Generally pitch it as, we are studying
% a myopic methods because they are feasible.
% And we will analyse when this works. Say that this is similar to what the
% submodularity guys are doing.
% \item Related work, 
% Here are some
% ~\citet{chen2017near,gabillon2013adaptive,gabillon2014large} \\
% But discuss other papers that you think are
% relevant. I don't really know what many of them are doing
% \item Can you take a pass through the theory section?
% \end{enumerate}
% }


==> archive/method_apr_28.tex <==

\section{Set up and Method}

In our formulation, the design problem is characterised by a parameter
$\theta\in\Theta$.
At time $t$, the decision maker is allowed to choose an action $\Xt$ in some domain
$\Xcal$ and in doing so observes $\YXt\in\Ycal$ drawn from $\PP(\cdot|\Xt,\thetatrue)$.
Here the distribution $\PP(Y|X,\theta)$ is assumed known.
% We will use $\PPj$ to denote distributions when conditioned on $\dataj$
% 
We will denote $\Dcalt$ to be the set of all sequences of $t$ action-observation pairs,
i.e. $\Dcalt = \{ \{(\Xj,\Yj)\}_{j=1}^t: \Xj\in\Xcal, \Yj\in\Ycal\}$.

A policy is a sequence of actions $\{\Xj\}_{j\in\NN}$ where $\Xt$ can depend on
past actions and observations, $\datatmo = \{(\Xj,\YXj)\}_{j=1}^{t-1}$.
In particular, for a \emph{randomised} policy $\policy = \{\policyj\}_{j\in\NN}$,
at time $t$, an action is drawn from
$\policyt(\datatmo) = \PP(\Xt\in\cdot|\datatmo)$.

We adopt the Bayesian paradigm and assume $\thetatrue$ itself is drawn from some
prior $\pthetazero$.


Let $\penlt:\Theta\times\Dcalt\rightarrow[0,1]$ be the penalty function in our design
problem.
Our goal in Bayesian design experiment design is to choose actions so as to minimise
$\penlt(\thetatrue,\datat)$ which depends on the true parameter and actions and
observations.
In particular, we are interested in the cumulative and final regrets, defined below.
\begin{align*}
\crn &= \sum_{t=1}^n \penlt(\thetatrue, \datat)\, -\, 
        \sum_{t=1}^n \penlt(\thetatrue, \ordatat)\\
\label{eqn:regretDefn}\numberthis
\frn &= \penln(\thetatrue, \datan)\, -\, \penln(\thetatrue, \ordatan)
\end{align*}
Here, $\ordatat = \argmin_{\datat\in\Dcalt} \EE\left[\penlt(\thetatrue,\datat)\right]$
is data chosen, possibly adaptively,
to minimise the expected penalty
by an oracle which knows the true parameter $\thetatrue$ ahead of time.
The expectation in $\ordatan$ is with respect to the randomness in the observations
$\PP(Y|X,\thetatrue)$.
The regrets in~\eqref{eqn:regretDefn} are random quantities, so we consider the
Bayesian regrets $\bcrn = \EE[\crn]$, $\bfrn = \EE[\frn]$ where the expectation
is over the prior $\pthetazero$, the observations, and any randomness in the
algorithm.

\textbf{Notation:}
$\PP,\EE$ denote probabilities and expectations.
$\PPt,\EEt$ denote probabilities and expectations when conditioned on
the actions and observations up to time $j$, e.g. for any event $E$, $\PPt(E) =
\PP(E|\datat)$.
$\pthetat$ denotes the posterior for $\thetatrue$ when conditioned on $\datat$,
$\pthetat(\cdot) = \PP(\thetatrue\in\cdot|\datat)$.

\subsection*{Algorithm}

We will first define the expected look-ahead penalty at time $t$,
$\penlplustmo:\Theta\times\Dcaltmo\times\Xcal\rightarrow[0,1]$ to be the
expected penalty at the next time step if $\theta\in\Theta$ were the true parameter and
we were to query at $x\in\Xcal$.
Precisely,
\begin{align*}
\penlplustmo(\theta,\Dcaltmo,x) \;=\; \EE_{\Yx\sim\PP(Y|x,\theta)}
\Big[\penlt\big(\theta,\,\Dcaltmo\cup\{(x, \Yx)\}\,\big) \Big]
\numberthis
\label{eqn:lookaheadpenalty}
\end{align*}

\insertAlgoMain


==> archive/method_may_20.tex <==

\section{Set up and Method}
\label{sec:method}

Let $\Theta$ denote a parameter space, $\Xcal$ an action space and
$\Ycal$ an outcome space.  We consider a Bayesian setting where a
\emph{true parameter} $\thetatrue \in \Theta$ is drawn from a prior
distribution $\pthetazero$. A decision maker repeatedly chooses an
action $X \in \Xcal$, conducts an experiment at $X$ and observes the
outcome $\YX \in\Ycal$. We assume $\YX$ is drawn from a
\emph{likelihood} $\PP(\cdot|X,\thetatrue)$, with known distributional
form. This process proceeds for $n$ rounds, resulting in a
\emph{data
sequence} $\dataseqn = \{(\Xj,\YXj)\}_{j=1}^n$, which is an ordered
multi-set of action-observation pairs. With $\Dcalseq$ denoting the
set of all possible data sequences, the goal is to minimize a
\emph{penalty function} $\penl: \Theta\times\Dcalseq\rightarrow[0,1]$,
and in particular, we focus on the following two criteria, depending
on the application:
%  that depends
% both on the true parameter and the collected data sequence. Depending
% on the application, we focus on the following two quantities:
\begin{align*}
\cridx\;\;
\sumpenl(\thetatrue, \datan) = \sum_{t=1}^n\penl(\thetatrue, \datat)
\hspace{1.0in}
% {\rm \bf (ii)}\;\;
\fridx\;\;
\penl(\thetatrue, \datan),
\label{eqn:penldefn} \numberthis
\end{align*}
Here $\datat=\{(\Xj,\YXj)\}_{j=1}^t$
denotes the prefix of length $t$ of the data sequence
$\datan$ collected by the decision maker.
The former notion is the
cumulative sum of all penalties, while the latter corresponds just to
the penalty once all experiments have been completed. Note that since
the penalty function depends on the unknown true parameter
$\thetatrue$, the decision maker cannot compute the penalty during the
data collection process, and instead must infer the penalty from
observations in order to minimise it. This is a key distinction from
existing work on reinforcement learning and sequential optimisation,
and one of the new challenges in our setting.


% In the former case, at time $t$, the decision maker chooses an action
% and incurs a penalty
% $\penl(\thetatrue, \dataseqtmo \cup \{(\Xt, \YXt)\})$.  The total
% penalty is the cumulative sum of all penalties.  In the latter, we are
% only interested in achieving a small penalty at the end of all
% experiments.  One of the key challenges, when compared to existing
% work in online learning, reinforcement learning and set function
% optimisation is that we do not directly observe the penalty (or a
% noisy version of it), since $\thetatrue$ is not known.  Instead, the
% decision maker needs to infer the penalty from the observations
% collected and work to minimise it.  For example, in active learning,
% one cannot compute the true penalty since $\tau_\star$ is not known
% (as that would render the whole exercise meaningless).

\insertprethmspacing
\begin{example}
  A motivating example is \emph{Bayesian active
    learning}~\cite{golovin2010near,chen2017near}. Here actions $X$
  correspond to data points while $\YX$ is the label and
  $\PP(y|x,\theta)$ specifies an assumed discriminative model. We
  may set
  $\penl(\theta,\datan) = \|\tau(\theta)-\hat{\tau}(\datan)\|_2^2$
  where $\tau$ is a parameter of interest and $\hat{\tau}$ is a
  predetermined estimator (e.g. maximum likelihood or maximum a posteriori).
  The true penalty
  $\penl(\thetatrue,\datan)$ is
  not available to the decision maker since it requires knowing
  $\tau(\thetatrue)$.
\end{example}

% Let $\Theta$ be a set.
% In our formulation, the design problem is characterised by a \emph{true parameter}
% $\thetatrue\in\Theta$.
% We adopt the Bayesian paradigm where $\thetatrue$ is assumed to be drawn from some
% prior $\pthetazero$.
% A decision maker can choose an action $X$ in some domain $\Xcal$.
% Then, an experiment is conducted at $X$,
% and the result (observation) $\YX\in\Ycal$
% % drawn from $\PP(\cdot|X,\thetatrue)$,
% is shown to the decision maker.
% $\YX$ is drawn from $\PP(\cdot|X,\thetatrue)$,
% and the form of the distribution $\PP(y|x,\theta)$ is assumed known.
% For example, in active learning, an action $X$ is a data point,
% $\YX$ is the label for $X$, and $\PP(y|x,\theta)$ specifies the discriminative
% model for the label.


\paragraph{Notation:} 
For each $t \in \NN$, let
$\Dcalseqt = \{\{(\Xj,\YXj)\}_{j=1}^t: \Xj\in\Xcal, \YXj\in\Ycal\}$
denote the set of all data sequences of length $t$, so that
$\Dcalseq = \bigcup_{t\in\NN}\Dcalseqt$.  We use $|D|$ to denote the
length of a data sequences and $D \concat D'$ for the concatenation of
two sequences.  $D \dssubset D'$ and $D' \dssupset D$ both equivalently denote
that $D$ is a prefix of $D'$. Given a data sequence $\dataseqt$, we
use $\dataseqtt{t'}$ for $t' < t$ to denote the prefix of the first
$t'$ action-observation pairs.


% In the design of experiments, we wish to collect a sequence of data,
% in the form of action-observation pairs $(X,Y)$ in order to 
% fulfil a certain objective.
% For instance, in active learning, our goal might be to estimate a parameter
% $\tau_\star = \tau(\theta_\star)$ of the data generating model.
% We will call an ordered multi-set of action-observation pairs
% $\dataseqt = \{(\Xj,\YXj)\}_{j=1}^{t}$ to be a \emph{data sequence}
% -- i.e. an element $(\Xj,\YXj)$ can be repeated in $\dataseqt$ and each data sequence
% is distinguished based on its ordering.
% This subsumes settings where the order of the data collected does not matter, i.e. sets or
% multi-sets.
% $\Dcalseqt$ will denote the set of all data sequences of length $t$,
% i.e. $\Dcalseqt = \{ \{(\Xj,\Yj)\}_{j=1}^t: \Xj\in\Xcal, \Yj\in\Ycal\}$,
% and
% $\Dcalseq = \bigcup_{t\in\NN}\Dcalseqt$ will be the union of all $\Dcalseqt$'s.
% Let $D, D'$ be two data sequences.
% We let $|D|$ be the length of $D$ and  $D\concat D'$ be the concatenation of
% $D$ and $D'$.
% $D\dssubset D'$ and $D'\dssupset D$ both equivalently
% mean that $D$ is a subsequence of $D'$ from
% the first $(X, Y)$ pair to the $|D|$\ssth.
% Given a data sequence $\dataseqt$ as defined above, when $t'<t$,
% we will denote the by $\dataseqtt{t'} = \{(\Xj,\YXj)\}_{j=1}^{t'}$, the first $t'$
% action observation pairs.
% Hence, $\dataseqtt{t'}\dssubset \dataseqt$ for all $t'< t$.
% When $\dataseqt\in\Dcalt$, we will use $\datat$ to denote the same multi-set but when
% the ordering does not matter.
% Similarly, $\Dcalt, \Dcalseqt$

% Our goal in Bayesian design of experiments is to choose actions so as to minimise
% a given \emph{penalty function}
% $\penl(\thetatrue,\dataseqt)$ which depends on the true parameter $\thetatrue$ and the
% data sequence $\datat$ collected by us.
% We will assume $\penl:\Theta\times\Dcalseq\rightarrow[0,1]$ and that $\penl(\emptyset) =
% 1$.
% In the active learning example, one might use
% $\penl(\theta, \datan) = \|\tau(\theta) - \hat{\tau}(\datan)\|_2^2$ where
% $\hat{\tau}$ is a pre-determined estimator for $\tau$ obtained from the data.
% The goal is to minimise the true penalty $\|\tau_\star - \hat{\tau}(\datan)\|_2^2$.
% The goal of a decision maker is to collect data so that $\penl$ is small.
% After $n$ experiments, and having collected a data sequence $\datan$,
% we might be interested in achieving small values to one of the following two
% quantities, depending on the application.
% \begin{align*}
% % {\rm \bf (i)}\;\;
% \cridx\;\;
% \sumpenl(\thetatrue, \datan) = \sum_{t=1}^n\penl(\thetatrue, \datat)
% \hspace{0.5in}
% % {\rm \bf (ii)}\;\;
% \fridx\;\;
% \penl(\thetatrue, \datan)
% \label{eqn:penldefn} \numberthis
% \end{align*}
% In the former case,
% at time $t$, the decision maker chooses an action and incurs a penalty 
% $\penl(\thetatrue, \dataseqtmo \cup \{(\Xt, \YXt)\})$.
% The total penalty is the cumulative sum of all penalties.
% In the latter, we are only interested in achieving a small penalty at the
% end of all experiments.
% One of the key challenges, when compared to existing work in online
% learning, reinforcement learning and set function optimisation is that we do not
% directly observe the
% penalty (or a noisy version of it), since $\thetatrue$ is not known.
% Instead, the decision maker needs to infer the penalty from the observations
% collected and work to minimise it.
% For example, in active learning, one cannot compute the true penalty
% since $\tau_\star$ is not known (as that would render the whole exercise meaningless).

A \emph{policy} for experiment design chooses a sequence of actions
$\{\Xj\}_{j\in\NN}$ based on past actions and observations.
% where $\Xt$ can depend on
% past actions and observations, $\dataseqtmo = \{(\Xj,\YXj)\}_{j=1}^{t-1}$.
In particular, for a \emph{randomised} policy
$\policy = \{\policyj\}_{j\in\NN}$, at time $t$, an action is drawn
from $\policyt(\dataseqtmo) = \PP(\Xt\in\cdot|\dataseqtmo)$. 
Two policies that will appear frequently in the sequel are $\gopolicy$ and
$\uopolicy$, both of which operate with knowledge of
$\thetatrue$. $\gopolicy$ is the myopic optimal policy, which, from
every data sequence $\datat$ chooses the action $X$ minimizing the expected penalty
at the next step: $\EE[\penl(\thetatrue,\datat\concat\{(X,\YX)\})|\thetatrue]$. On
the other hand $\uopolicy$ is the non-myopic, globally optimal policy,
which in state $\datat$ with $n-t$ steps to go chooses the action to
minimise the expected long-term penalty:
$\EE[\penl(\thetatrue,\datat\concat\{(X,\YX)\}\concat \datatt{t+2:n}) \mid
\uopolicy,\thetatrue]$.
% \akshay{Describe optimal policies here.}  
% \akshay{Also might I suggest
%   less confusing names for the optimal policies. If you are not using
%   subscripts on them, can we say $\pi_M^\star$ and $\pi_G^\star$?}

% 
% 

% In particular, for a policy $\pi$


\subsection*{Design of Experiments via Posterior Sampling}

We present a simple and intuitive myopic strategy that aims to minimise $\penl$ based on
the posterior of the data collected so far.
For this, first define the expected look-ahead penalty %at time $t$,
$\penlplus:\Theta\times\Dcal\times\Xcal\rightarrow[0,1]$ to be the
expected penalty at the next time step if $\theta\in\Theta$ were the true parameter and
we were to take action $x\in\Xcal$.
Precisely, for a data sequence $D$,
\begin{align*}
\penlplus(\theta,D,x) \;=\; \EE_{\Yx\sim\PP(Y|x,\theta)}
\Big[\penlt\big(\theta,\,D\concat\{(x, \Yx)\}\,\big) \Big].
\numberthis
\label{eqn:lookaheadpenalty}
\end{align*}
The proposed policy, presented in Algorithm~\ref{alg:bdoe},
is called \bdoes (Myopic Posterior Sampling) and is denoted $\pspolicy$.
At time step $t$,
it first samples a parameter value $\theta$ from the posterior  for
$\thetatrue$ conditioned on the data, i.e. $\theta\sim\PP(\thetatrue|\datatmo)$.
Then, it chooses the action $\Xt$ that is expected to minimise the penalty $\penl$ by
pretending that $\theta$ was the true parameter.
It performs the experiment at $\Xt$, collects the observation $\YXt$, and proceeds to the 
next time step.
% keeps repeating
% this routine on each iteration.


\insertAlgoMain

\textbf{Computational considerations:}
It is worth pointing out some of the computational considerations in
Algorithm~\ref{alg:bdoe}.
First, sampling from the posterior for $\thetatrue$ in step~\ref{step:sampletheta}
might be difficult, especially in complex Bayesian models.
Fortunately however, the field of Bayesian inference has made great strides in the recent
past seeing the development of fast techniques for approximate inference methods such as
MCMC or variational inference.
Moreover, today we have efficient probabilistic programming
tools~\citep{carpenter2017stan,tran2017edward} that allow a practitioner to intuitively
incorporate domain expertise via a prior and obtain the posterior given data.
Secondly, the minimisation of the look ahead penalty in step~\ref{step:choosext}
can also be non-trivial, especially since it might involve empirically computing
the expectation in~\eqref{eqn:lookaheadpenalty}.
This is similar to existing work in Bayesian optimisation which assume access to such an
optimisation
oracle~\citep{srinivas10gpbandits,bull11boRates}.
That said, in many practical settings where experiments are  financially expensive and
can take several hours, these considerations are less critical.
% can take hours and involve

% , these considerations may not be significant.
% For example, in many industrial DOE problems, an experiment might require several
% hours and involve significant monetary cost.
% In such settings, one cares more about incorporating domain expertise in a possibly
% complex model, over developing computationally efficient algorithm


Despite these concerns, it is worth mentioning that myopic strategies are
still computationally far more attractive than policies which try to behave globally
optimally.
For example, extending \mpss to a $k$ step look-ahead might involve an optimisation
over $\Xcal^k$ in step~\ref{step:choosext} of Algorithm~\ref{alg:bdoe} which might
be impractical for large values of $k$ except in the most trivial settings.


\textbf{Specification of the prior:}
In real world applications, the prior could be specified by a domain expert with knowledge
of the given DOE problem.
In some instances, the expert may only be able to specify the relations between the
various variables involved.
In such cases, one can specify the parametric form for the prior, and learn the
parameters of the prior in an adaptive data dependent fashion using maximum likelihood
and/or maximum a posteriori techniques~\citep{snoek12practicalBO}.
While we adopt both approaches in our experiments, we assume a fixed prior in our
theoretical analysis.

% For what follows, we will define $\gopolicy$ to be a policy which \emph{knows}
% $\thetatrue$ and behaves in a myopically optimal manner and collects
% $\godatan$ in $n$ steps.
% % and collects $\godatan$.
% % That is, if $\godatat$ to be the data collected by this policy  in $t$ steps.
% That is $\gopolicy$ follows Algorithm~\ref{alg:bdoe}
% but skips line~\ref{step:sampletheta} and
% in step~\ref{step:choosext} uses $\thetatrue$ instead of a sampled $\theta$ value.
% Further, step~\ref{step:initdata} is replaced with $\godatatt{0}\leftarrow\emptyset$ and
% step~\ref{step:adddata} with $\godatat\leftarrow\godatatmo\concat\{(\Xt,\Yt)\}$.
% For example,
% in active learning, $\gopolicy$ will know the true parameter $\thetatrue$
% and will attempt to collect data to minimise $\|\tau_\star - \hat{\tau}(\datan)\|$.
% $\gopolicy$ will be integral to our theoretical analysis of
% $\pspolicy$ in Section~\ref{sec:regret}.
% Further, while it is not realisable in practice since it assumes knowledge of 
% $\thetatrue$, it still provides a good benchmark for empirical comparison.




==> archive/proofs_may5.tex <==

\section{Proofs}

\subsection{Notation and Set up}

In this subsection, we will introduce some notation, prove some basic lemmas
and in general, lay the groundwork for our analysis.
% This includes some basic lemmas and


% \textbf{Notation:}
$\PP,\EE$ denote probabilities and expectations.
$\PPt,\EEt$ denote probabilities and expectations when conditioned on
the actions and observations up to and including
time $t$, e.g. for any event $E$, $\PPt(E) = \PP(E|\datat)$.
For two data sequences $A,B$, $A\concat B$ denotes the concatenation of the two
sequences.
% $\pthetat$ denotes the posterior for $\thetatrue$ when conditioned on $\datat$,
% $\pthetat(\cdot) = \PP(\thetatrue\in\cdot|\datat)$.
% 
% We will introduce some notation before we proceed.
Let $\datat\in\Dcalt$ be a data sequence of length $t$.
Then, $\Qpi(\datat,x)$ will denote the expected total penalty when we take action
$x$ and then execute policy $\policy$ for the remaining $n-t-1$ steps.
That is,
\begin{align*}
\numberthis\label{eqn:Qdefn}
&\Qpi(\datat, x) = \EE\big[\sumpenl(\thetatrue, \datat\concat\{(x, \Yx)\}\cup\Ftptn) \big] \\
&\hspace{0.05in}
= \sum_{j=1}^t\penl(\thetatrue, \dataj) +
  \EE_{\Yx, \Ftptn}\bigg[\penl(\thetatrue, \dataj\concat\{(x,\Yx)\})
%   &\hspace{0.3in}
  + \sum_{j=t+2}^n \penl(\thetatrue, \dataj\concat\{(x,\Yx)\}\cup
      \Fttnn{t+2}{j} ) \bigg]
\end{align*}
Here, the action-observation pairs collected by $\policy$
from steps $t+2$ to $n$ are $\Ftptn$.
The expectation is over the observations and any randomness in $\policy$.
While we have omitted for conciseness,
$\Qpi$ is a function of the true parameter $\thetatrue$.
Let $\dttpp{t}{\pi}$ denote the distribution of $\datat$ when following a policy $\pi$
for the first $t$ steps. % to be $\dttpp{t}{\pi}$.
We then have,
\begin{align*}
J(\thetatrue,\policy) = \EE_{\datat\sim\dttpp{t}{\policy}}
\big[\EE_{X\sim\policy(\datat)}[\Qpp{\policy}(\datat, X)]\big].
\numberthis \label{eqn:lossQ}
\end{align*}

The following Lemma, decomposes the regret~\eqref{eqn:regretDefn}
as a sum of terms which are convenient to analyse.
The proof is adapted from Lemma 4.3 in~\citet{ross2014reinforcement}.

\insertprethmspacing
\begin{lemma}
For any two policies $\policyone,\policytwo$,
\begin{align*}
&J(\thetatrue,\policyone) - J(\thetatrue,\policytwo) = \\
% = \sum_{t=1}^n \EE_{\datatmo \sim \dtmopo, X\sim\policyone(\datatmo)}\left[
%  \Qpt(\datatmo, X) \right]
%  -\EE_{\datatmo \sim \dtmopo, X\sim\policytwo(\datatmo)}\left[
%  \Qpt(\datatmo, X) \right]
&\hspace{0.4in} \sum_{t=1}^n \EE_{\datatmo \sim \dtmopo}\left[
  \EE_{X\sim\policyone(\datatmo)}\left[
 \Qpt(\datatmo, X) \right]
 -\EE_{X\sim\policytwo(\datatmo)}\left[
 \Qpt(\datatmo, X) \right]
  \right]
\end{align*}
\label{lem:valuedecomp}
\begin{proof}
Let $\policy^t$ be the policy that follows $\policyone$ from time step $1$ to $t$, and
then executes policy $\policytwo$ from $t+1$ to $n$.
Hence, by~\eqref{eqn:lossQ}, 
\[J(\thetatrue, \policy^t) 
=\; \EE_{\datatmo\sim\dttpp{t-1}{\policyone}}
\big[\EE_{X\sim\policyone(\datatmo)}[\Qpp{\policytwo}(\datatmo, X)]\big]
=\;
\EE_{\datat\sim\dttpp{t}{\policyone}}
\big[\EE_{X\sim\policytwo(\datat)}[\Qpp{\policytwo}(\datat, X)]\big]
\]
The claim follows from the observation,
$
J(\thetatrue, \policyone) - J(\thetatrue, \policytwo) =
J(\thetatrue, \policy^n) - J(\thetatrue, \policy^0) =
\sum_{t=1}^n J(\thetatrue, \policy^t) - J(\thetatrue, \policy^{t-1}).
$
% &\hspace{0.2in}
% = \sum_{t=1}^n J(\thetatrue, \policy^t) - J(\thetatrue, \policy^{t-1}) \\
\end{proof}
\end{lemma}

We will use Lemma~\ref{lem:valuedecomp} with $\policytwo$ as the policy $\gopolicy$
which knows $\thetatrue$ and with $\policyone$ as the policy $\policy$
whose regret we wish to bound.
For this, 
denote the action chosen by $\policy$ when it has seen data $\datatmo$
as $\Xt$.
%  and that taken by $\gopolicy$ as $\Xpt$. %, i.e. $\Xt\sim\policy(\datatmo)$
% and $\Xpt\sim\gopolicy(\datatmo)$.
Denote the action-observations pairs when choosing
$\Xt\sim\policy(\datatmo)$ and then following $\gopolicy$
as $\Htmotn$, i.e. $\Htmotn$ includes $(\Xt, \YXt)$ and has length $n-t+1$.
Similarly,  denote the action chosen by $\gopolicy$ when it has seen data $\datatmo$
as $\Xpt$ and the ensuing $n-t+1$ action-observations pairs when following
$\gopolicy$ as $\Hptmotn$.
By Lemma~\ref{lem:valuedecomp} and equation~\eqref{eqn:Qdefn} we have,
\begin{align*}
\EE_{\thetatrue}[\loss(\thetatrue,\policy) - \loss(\thetatrue,\gopolicy)]
&= \EE \sum_{t=1}^n \EEtmo\Big[
 \underbrace{\Qpp{\gopolicy}(\datatmo,\Xt)
 - \Qpp{\gopolicy}(\datatmo,\Xpt)}_{r_t} \Big] \\
% \underbrace{\Qpp{\gopolicy}(\datatmo,\Xt)
%  - \Qpp{\gopolicy}(\datatmo,\Xpt) }_{r_t}  \Big]
&= \EE \sum_{t=1}^n \EEtmo\Big[
\underbrace{\sumpenl(\datatmo\concat\Htmotn)
 - \sumpenl(\datatmo\concat\Hptmotn)}_{r_t} \Big] \\
\end{align*}
Note that $\EEtmo$, which conditions on $\datatmo$ collected by $\policy$,
encompasses three sources of randomness.
The first is due to the randomness in the problem due to $\thetatrue\sim\pthetazero$,
the second is due to the observations $Y\sim\PP(\cdot|X,\thetatrue)$,
and the third 
is an external source of randomness $U$ used by the decision maker in
step~\ref{step:sampletheta} in Algorithm~\ref{alg:bdoe}.
While the actions $\{\Xt\}_t$ chosen depends on all sources of randomness, these
three sources are themselves independent.
For example, we can write $\EEtmo[r_t] = \EEU[\EEtmorho[\EEtmoY[r_t]]]$
where $\EEU$ captures the randomness by the decision maker,
$\EEtmorho$ due to the prior
and
$\EEtmoY$ due to the observations.
With this in consideration, 
denote $\qt(x,y) = \EEtt{Y,t+1:n}[\Qpp{\gopolicy}(\datatmo,x,y)]$
to be the expected total penalty when we
have data $\datatmo$ collected by $\policy$, then execute action $x$ at time $t$,
observe $y$ and then execute $\gopolicy$.
We then have,
\begin{align*}
\EE_{\thetatrue}[\loss(\thetatrue,\policy) - \loss(\thetatrue,\gopolicy)]
&= \EE \sum_{t=1}^n \EEtmo\Big[
  \qt(\Xt, \YXt) - \qt(\Xpt, \YXpt)
  \Big], \\
\end{align*}
where $\EEtmo$ captures the randomness in $U,\rho$ and the
observations at time $t$.

\toworkon{check notation with various randomness!}

\insertprethmspacing
\begin{proof}


Finally, for the purposes of the analysis, we will allow a decision maker to take
no action at any given time step $t$ and denote this by $\emptyset$,
i.e. $\datat\concat\emptyset\cup\Ftptn$ means the action observation pairs were
$\datat$ from time $1$ to $t$, then there was no action at time $t+1$ and then
from time $t+2$ to $n$, the action observation pairs were $\Ftptn$.
In doing so, the decision maker incurs a penalty of $\penl(\thetatrue,\datat)$
at step $t+1$.
% In doing so, the decision maker incurs a (maximum) penalty of $1$ at step $t+1$.
% \toworkon{the penalty can also be $\penl(\thetatrue,\datat)$}.
\toworkon{the penalty can also be $1$}.
Correspondingly, we have,
\begin{align*}
\sumpenl(\thetatrue,\datat\concat\emptyset\cup\Ftptn)
 = \sum_{j=1}^t\penl(\thetatrue,\dataj) + \penl(\thetatrue,\datat)
  + \sum_{j=t+2}^n\penl(\thetatrue,\datat\concat\Fttnn{t+2}{j})
\end{align*}

We will now argue $\EEtmoY[r_t] \leq 1$.
Adding and subtracting $
\sumpenl(\thetatrue, \datatmo\concat\emptyset\cup\Hptmotnmo)\big)
$ we have,
% Writing
\begin{align*}
r_t =\;&
\big(\sumpenl(\thetatrue, \datatmo\concat\Htmotn)  -
\sumpenl(\thetatrue, \datatmo\concat\emptyset\cup\Hptmotnmo)\big)
\;+ \\
&
\big(
\sumpenl(\thetatrue, \datatmo\concat\emptyset\cup\Hptmotnmo) - 
\sumpenl(\thetatrue, \datatmo\concat\Hptmotn)
\big).
\end{align*}
The second term above can be bounded by $1$ since $\lambda$ maps to $[0,1]$.
\begin{align*}
&\sumpenl(\thetatrue, \datatmo\concat\emptyset\cup\Hptmotnmo) - 
\sumpenl(\thetatrue, \datatmo\concat\Hptmotn) \\
&\hspace{0.3in} =
\penl(\thetatrue,\datatmo) + \sum_{j=t+1}^{n-1}\penl(\thetatrue,\datatmo\concat\Hptmotj)
                           - \sum_{j=t+1}^{n}\penl(\thetatrue,\datatmo\concat\Hptmotj) \\
&\hspace{0.3in} =
 \penl(\thetatrue,\datatmo) - \penl(\thetatrue, \datatmo\concat\Hptmotn) \leq 1.
\end{align*}
For the first term, we similarly have,
\begin{align*}
% \EEtmoY\big[
&\big(\sumpenl(\thetatrue, \datatmo\concat\Htmotn)  -
\sumpenl(\datatmo\concat\emptyset\cup\Hptmotnmo)\big) \\
&\hspace{0.2in}= 
  \big(\penl(\thetatrue, \datatmo\concat\{(\Xt,\YXt)\}) -  \penl(\thetatrue, \datatmo)\big)
  \;+\;
\\
&\hspace{0.5in}
  \sum_{j=t+1}^n\big(\penl(\thetatrue, \datat\concat\Htmotj) -
                \penl(\thetatrue, \datat\concat\Hptmotjmo)\big).
\end{align*}
We will show that each of $n-t+1$ terms in the RHS sum are non-positive in
expectation via an inductive argument.
We use the first term as the base step,
where we have,
$\EEtt{\YXt}[\penl(\thetatrue, \datatmo\concat\{(\Xt,\YXt)\})]
\leq \penl(\thetatrue, \datatmo)$ by the first monotonicity condition
in Condition~\ref{cond:monotonicity}.
For the inductive step, assume that
$\EEtmoY[\penl(\thetatrue, \datat\concat\Htmotj) -
         \penl(\thetatrue, \datat\concat\Hptmotjmo)] \leq 0$.
Then, by the second monotonicity condition,
$\EEtmoY[\penl(\thetatrue, \datat\concat\Htmotjpo) -
         \penl(\thetatrue, \datat\concat\Hptmotj)] \leq 0$.
% $r_t = \sumpenl(\datatmo\concat\Htmotn) - \sumpenl(\datatmo\cup\Hptmotnmo)
% +
We conclude the proof as follows,
\begin{align*}
\EEtmo[r_t] = \EEU[\EEtmorho[\EEtmoY[r_t]]]
\end{align*}
TBC.
\end{proof}

\begin{align*}
\EEtmo[r_t] &= \EEtmo\left[ \right]
\end{align*}

% We will define two quantities which we will need for our purpose.
% The first is the information ratio $\IRn$ and second is the maximum information gain
% $\IGn$.
% \begin{align*}
% \IRt &= \frac{\EEtmo[\penlt(\thetatrue,\datat) - \penlt(\thetatrue,\iodatat)]^2}{%
%  \Itmo(\thetatrue; (\Xt, \YXt)) }
% \numberthis\label{eqn:infratio}
%  \\
% \IGt &= \max_{\datat\subset\Dcalt} I(\thetatrue; \datat)
% \numberthis\label{eqn:mig}
% \end{align*}
% 
% \insertprethmspacing
% \begin{theorem}
% \label{prop:baseprop}
% For all $n\geq 0$, if $\IRt\leq\IRbar$ for all $t\leq n$, then,
% \emph{
% \[
% \EE[\crthrn] \leq
%   \sqrt{n\IRn\IGn}
% \]
% }
% \begin{proof}
% First using the quantities above and the Cauchy-Schwarz inequality we have,
% \begin{align*}
% \EE[\crthrn] \;&\leq\;
% \EE\sumoton\EEtmo[\penlt(\thetatrue,\datat) - \penlt(\thetatrue,\iodatat)]
% % \\
% \leq\; \sqrt{\IRbar}\left(\EE\sumoton\sqrt{\It(\thetatrue;(\Xt,\YXt))}\right)
% \\
% &\leq \sqrt{n\IRbar\sumoton\EE[\Itmo(\thetatrue;(\Xt,\YXt))]}.
% \end{align*}
% We conclude the proof with the following calculation which uses the chain rule for
% mutual information.
% \begin{align*}
% \sumoton \EE\Itmo(\thetatrue; (\Xt,\YXt)) =
% \sumoton I(\thetatrue; (\Xt, \YXt) | \datatmo) = I(\thetatrue; \datan) \leq \IGn.
% \end{align*}
% \end{proof}
% \end{theorem}
% 
% \toworkon{I can bound $\IRn$ using techniques in~\citet{russo2016thompson} and
% $\IGn$ using techniques in~\citet{srinivas10gpbandits}.}

\toworkon{
Simple regret with submodular functions.
}


==> archive/proofs_may_14.tex <==

\section{Proofs}

\subsection{Notation and Set up}

In this subsection, we will introduce some notation, prove some basic lemmas,
and in general, lay the groundwork for our analysis.
$\PP,\EE$ denote probabilities and expectations.
$\PPt,\EEt$ denote probabilities and expectations when conditioned on
the actions and observations up to and including
time $t$, e.g. for any event $E$, $\PPt(E) = \PP(E|\datat)$.
For two data sequences $A,B$, $A\concat B$ denotes the concatenation of the two
sequences.
When $x\in\Xcal$, $\Yx$ will denote the random observation from
$\PP(Y|x,\theta)$.

% $\pthetat$ denotes the posterior for $\thetatrue$ when conditioned on $\datat$,
% $\pthetat(\cdot) = \PP(\thetatrue\in\cdot|\datat)$.
% 
% We will introduce some notation before we proceed.
Let $\datat\in\Dcalt$ be a data sequence of length $t$.
Then, $\Qpi(\datat,x,y)$ will denote the expected total penalty when we take action
$x\in\Xcal$, observe $y\in\Ycal$ and then execute policy $\policy$ for the remaining
$n-t-1$ steps.
That is,
\begin{align*}
\numberthis\label{eqn:Qdefn}
&\Qpi(\datat, x, y) = \EE\big[\sumpenl(\thetatrue, \datat\concat\{(x, y)\}\concat\Ftptn) \big] \\
&\hspace{0.05in}
= \sum_{j=1}^t\penl(\thetatrue, \dataj) +
  \penl(\thetatrue, \dataj\concat\{(x,y)\}) +
  \EE_{\Ftptn}\bigg[
  \sum_{j=t+2}^n \penl(\thetatrue, \dataj\concat\{(x,y)\}\concat
      \Fttnn{t+2}{j} ) \bigg].
\end{align*}
Here, the action-observation pairs collected by $\policy$
from steps $t+2$ to $n$ are $\Ftptn$.
The expectation is over the observations and any randomness in $\policy$.
While we have omitted for conciseness,
$\Qpi$ is a function of the true parameter $\thetatrue$.
Let $\dttpp{t}{\pi}$ denote the distribution of $\datat$ when following a policy $\pi$
for the first $t$ steps. % to be $\dttpp{t}{\pi}$.
We then have,
\begin{align*}
J(\thetatrue,\policy) = \EE_{\datat\sim\dttpp{t}{\policy}}
\big[
\EE_{X\sim\policy(\datat)}[
%      \EE_{\YX\sim\PP(Y|X,\thetatrue)}[
  \Qpp{\policy}(\datat, X, Y)]\big],
\numberthis \label{eqn:lossQ}
\end{align*}
where, recall, $\YX$ is drawn from $\PP(Y|X,\thetatrue)$.
The following Lemma decomposes the regret~\eqref{eqn:regretDefn}
as a sum of terms which are convenient to analyse.
The proof is adapted from Lemma 4.3 in~\citet{ross2014reinforcement}.

\insertprethmspacing
\begin{lemma}
For any two policies $\policyone,\policytwo$,
\begin{align*}
&J(\thetatrue,\policyone) - J(\thetatrue,\policytwo) = \\
% = \sum_{t=1}^n \EE_{\datatmo \sim \dtmopo, X\sim\policyone(\datatmo)}\left[
%  \Qpt(\datatmo, X) \right]
%  -\EE_{\datatmo \sim \dtmopo, X\sim\policytwo(\datatmo)}\left[
%  \Qpt(\datatmo, X) \right]
&\hspace{0.2in} \sum_{t=1}^n \EE_{\datatmo \sim \dtmopo}\left[
  \EE_{X\sim\policyone(\datatmo)}\left[
 \Qpt(\datatmo, X, \YX) \right]
 -\EE_{X\sim\policytwo(\datatmo)}\left[
 \Qpt(\datatmo, X, \YX) \right]
  \right]
\end{align*}
\label{lem:valuedecomp}
\begin{proof}
Let $\policy^t$ be the policy that follows $\policyone$ from time step $1$ to $t$, and
then executes policy $\policytwo$ from $t+1$ to $n$.
Hence, by~\eqref{eqn:lossQ}, 
\begin{align*}
J(\thetatrue, \policy^t) &=
\; \EE_{\datatmo\sim\dttpp{t-1}{\policyone}}
\big[\EE_{X\sim\policyone(\datatmo)}[\Qpp{\policytwo}(\datatmo, X, \YX)]\big] \\
&=\;
\EE_{\datat\sim\dttpp{t}{\policyone}}
\big[\EE_{X\sim\policytwo(\datat)}[\Qpp{\policytwo}(\datat, X, \YX)]\big].
\end{align*}
The claim follows from the observation,
$
J(\thetatrue, \policyone) - J(\thetatrue, \policytwo) =
J(\thetatrue, \policy^n) - J(\thetatrue, \policy^0) =
\sum_{t=1}^n J(\thetatrue, \policy^t) - J(\thetatrue, \policy^{t-1}).
$
% &\hspace{0.2in}
% = \sum_{t=1}^n J(\thetatrue, \policy^t) - J(\thetatrue, \policy^{t-1}) \\
\end{proof}
\end{lemma}

We will use Lemma~\ref{lem:valuedecomp} with $\policytwo$ as the policy $\gopolicy$
which knows $\thetatrue$ and with $\policyone$ as the policy $\policy$
whose regret we wish to bound.
For this, 
denote the action chosen by $\policy$ when it has seen data $\datatmo$
as $\Xt$ and that taken by $\gopolicy$ as $\Xpt$. %, i.e. $\Xt\sim\policy(\datatmo)$
% For this, 
% denote the action chosen by $\policy$ when it has seen data $\datatmo$
% as $\Xt$.
% Denote the action-observations pairs when choosing
% $\Xt\sim\policy(\datatmo)$ and then following $\gopolicy$
% as $\Htn$, i.e. $\Htn$ includes $(\Xt, \YXt)$ and has length $n-t+1$.
% Similarly,  denote the action chosen by $\gopolicy$ when it has seen data $\datatmo$
% as $\Xpt$ and the ensuing $n-t+1$ action-observations pairs when following
% $\gopolicy$ as $\Hptmotn$.
By Lemma~\ref{lem:valuedecomp} and equation~\eqref{eqn:Qdefn} we have,
\begin{align*}
% \EE_{\thetatrue}[\loss(\thetatrue,\policy) - \loss(\thetatrue,\gopolicy)]
% &= \sum_{t=1}^n \EEtmo\Big[
%  \underbrace{\Qpp{\gopolicy}(\datatmo,\Xt,\YXt)
%  - \Qpp{\gopolicy}(\datatmo,\Xpt,\YXpt)}_{r_t} \Big] \\
% % \underbrace{\Qpp{\gopolicy}(\datatmo,\Xt)
% %  - \Qpp{\gopolicy}(\datatmo,\Xpt) }_{r_t}  \Big]
% &= \sum_{t=1}^n \EEtmo\Big[
% \underbrace{\sumpenl(\datatmo\concat\Htn)
%  - \sumpenl(\datatmo\concat\Hptmotn)}_{r_t} \Big]
\EE_{\thetatrue}[\loss(\thetatrue,\policy) - \loss(\thetatrue,\gopolicy)]
&= \sum_{t=1}^n \EEtmo\Big[
 \Qpp{\gopolicy}(\datatmo,\Xt,\YXt)
 - \Qpp{\gopolicy}(\datatmo,\Xpt,\YXpt) \Big]. %\\
% \underbrace{\Qpp{\gopolicy}(\datatmo,\Xt)
%  - \Qpp{\gopolicy}(\datatmo,\Xpt) }_{r_t}  \Big]
% &= \sum_{t=1}^n \EEtmo\Big[
% \underbrace{\sumpenl(\datatmo\concat\Htn)
%  - \sumpenl(\datatmo\concat\Hptmotn)}_{r_t} \Big]
\end{align*}
Note that $\EEtmo$, which conditions on the data sequence
$\datatmo$ collected by $\policy$,
encompasses three sources of randomness.
The first is due to the randomness in the problem due to $\thetatrue\sim\pthetazero$,
the second is due to the observations $Y\sim\PP(\cdot|X,\thetatrue)$,
and the third 
is an external source of randomness $U$ used by the decision maker in
step~\ref{step:sampletheta} in Algorithm~\ref{alg:bdoe}.
While the actions $\{\Xt\}_t$ chosen depends on all sources of randomness, these
three sources are themselves independent.
For example, we can write $\EEtmo[\cdot] = \EEU[\EEtmorho[\EEtmoY[\cdot]]]$
where $\EEU$ captures the randomness by the decision maker,
$\EEtmorho$ due to the prior
and
$\EEtmoY$ due to the observations.
With this in consideration, 
define
\begin{align*}
\qt(x,y) = \EEtt{Y,t+1:n}[\Qpp{\gopolicy}(\datatmo,x,y)],
\numberthis
\label{eqn:qtdefn}
\end{align*}
where $\EEtt{Y,t+1:n}$ is the expectation over the observations from time step
$t+1$ to $n$.
$\qt$ is the expected total penalty when we
have data $\datatmo$ collected by $\policy$, then execute action $x$ at time $t$,
observe $y$ and then follow $\gopolicy$ for the remaining time steps.
Note that $\qt$ is a deterministic function of $\thetatrue$, $x$, and $y$
since $\gopolicy$ is a deterministic policy and the randomness of future observations
has been integrated out.
We can now write,
\begin{align*}
\EE[\loss(\thetatrue,\policy) - \loss(\thetatrue,\gopolicy)]
&= \sum_{t=1}^n \EEtmo\Big[
  \qt(\Xt, \YXt) - \qt(\Xpt, \YXpt)
  \Big],
\numberthis
\label{eqn:lossqt}
\end{align*}
where $\EEtmo$ inside the summation is over the randomness in $\thetatrue$,
the randomness of the policy in choosing $\Xt$ and
the observations $\YXt, \YXpt$.

\subsection{Proof of Theorem~\ref{thm:finiteactions}}

We will let $\Ptildetmo$ denote the distribution of $\Xt$ given $\datatmo$;
i.e. $\Ptildetmo(\cdot) = \PPtmo(\Xt=\cdot)$.
The density (Radon-Nikodym derivative) $\ptildetmo$ of $\Ptildetmo$ can be expressed as
$\ptildetmo(x) = \int_\Theta p_{\star}(x|\theta)p(\theta|\datatmo)\ud \theta$
where $p_\star(x|\theta)$ is the density of the maximiser given $\theta$
and $p(\theta|\datatmo)$ is the posterior density of $\theta$ conditoned
on $\datatmo$.
Hence, $\Xt$ has the same distribution as $\Xpt$;
% i.e. $\Xt \stackrel{d}{=} \Xpt$.
i.e. $\PPtmo(\Xpt=\cdot) = \Ptildetmo(\cdot)$. % \stackrel{d}{=} \Xpt$.
This will form a key intuition in our analysis.
To this end, 
we begin with a technical result, whose proof is adapted from~\citet{russo2016thompson}.
We will denote by $\MItmo(A;B)$ the mutual information between two variables
$A,B$ under the posterior measure after having seen $\datatmo$;
i.e. $\MItmo(A;B) = \KL(\PPtmo(A,B)\|\PPtmo(A)\cdot\PPtmo(B))$.

\insertprethmspacing
\begin{lemma}
\label{lem:russolemmas}
Assume that we have collected a data sequence $\datatmo$.
Let the action taken by $\pspolicy$ with $\datatmo$ be $\Xt$ and the action taken by
$\gopolicy$ be $\Xpt$.
Let $\ptildetmo$ be the density of $\Xt$ given $\datatmo$.
Then,
\begin{align*}
&
\EEtmo[\qt(\Xt,\YXt) -  \qt(\Xpt,\YXpt)]
=\int_{x\in\Xcal} \hspace{-0.15in}
\big(\EEtmo[\qt(x,\Yx)] - \EEtmo[\qt(x,\Yx)|\Xpt=x]\big) \ptildetmo(x)  \ud x \\
&\MItmo(\Xpt; (\Xt, \YXt)) = \iint_{x_1,x_2\in\Xcal} \hspace{-0.30in}
  \KL(\PPtmo(\Yxone|\Xpt=x_2)\| \PPtmo(\Yxone) )\,
  \ptildetmo(x_1)\ptildetmo(x_2)\ud x_1\ud x_2
\end{align*}
\begin{proof}
The proof for both results uses the fact that
$\ud\PPtmo(\Xt=x) = \ud\PPtmo(\Xpt=x) = \ptildetmo(x)$.
For the first result,
\begin{align*}
&\EEtmo[\qt(\Xt,\YXt) -  \qt(\Xpt,\YXpt)] \\
&\hspace{0.1in} =
\int_{x\in\Xcal} \hspace{-0.15in}
\ud\PPtmo(\Xt=x)\EEtmo[\qt(\Xt,\YXt)|\Xt=x]
-
\int_{x\in\Xcal} \hspace{-0.15in}
\ud\PPtmo(\Xpt=x)\EEtmo[\qt(\Xpt,\YXpt)|\Xpt=x] \\
&\hspace{0.1in} =
\int_{x\in\Xcal} \hspace{-0.15in}
\ud\PPtmo(\Xt=x)\EEtmo[\qt(x,\Yx)]
- \int_{x\in\Xcal} \hspace{-0.15in} \ud\PPtmo(\Xpt=x)\EEtmo[\qt(x,\Yx)|\Xpt=x] \\
&\hspace{0.1in} =
\int_{x\in\Xcal} \hspace{-0.15in}
\big(\EEtmo[\qt(x,\Yx)] - \EEtmo[\qt(x,\Yx)|\Xpt=x]\big) \ptildetmo(x)  \ud x \,.
\end{align*}
The second step uses the fact that the observation $\Yx$ does not depend on
the fact that $x$ may have been chosen by $\pspolicy$;
this is because $\pspolicy$ makes its decisions based on past data $\datatmo$
and is independent of $\thetatrue$ given $\datatmo$.
$\Yx$ however can depend on the fact that $x$ may have been the action chosen by
$\gopolicy$ which knows $\thetatrue$.
For the second result,
\begin{align*}
&\MItmo(\Xpt; (\Xt, \YXt)) =
  \MItmo(\Xpt; \Xt) + \MItmo(\Xpt; \YXt|\Xt)
= \MItmo(\Xpt; \YXt|\Xt)
\\ &\hspace{0.1in} =
\int_{x_1\in\Xcal} \hspace{-0.20in} \ud\PPtmo(\Xt=x_1)\,\MItmo(\Xt;\YXt|\Xt=x)
=
\int_{x_1\in\Xcal} \hspace{-0.20in} \ptildetmo(x_1)\ud(x)\,\MItmo(\Xpt;\Yxone)
\\ &\hspace{0.1in} =
\int_{x_1\in\Xcal} \hspace{-0.20in} \ptildetmo(x_1)\ud(x)
\int_{x_2\in\Xcal} \hspace{-0.20in} \ud\PPtmo(\Xpt=x_2)
\,\KL(\PP(\Yxone|\Xpt=x_2)\|\PP(\Yxone))
\\ &\hspace{0.1in} =
  \iint_{x_1,x_2\in\Xcal} \hspace{-0.30in}
  \KL(\PPtmo(\Yxone|\Xpt=x_2)\| \PPtmo(\Yxone))\,
  \ptildetmo(x_1)\ptildetmo(x_2)\ud x_1\ud x_2
\end{align*}
The first step uses the chain rule for mutual information.
The second step uses that $\Xt$ is chosen based on an external source of randomness and
$\datatmo$;
therefore, it
is independent of $\thetatrue$ and hence $\Xpt$ given $\datatmo$.
The fourth step uses that $\Yxone$ is independent of $\Xt$.
The fifth step uses lemma~\ref{lem:klmi} in Appendix~\ref{app:ancillary}.
\end{proof}
\end{lemma}

The next Lemma uses the conditions on $\penl$ given in Section~\ref{sec:regret}
to show that $\qt$~\eqref{eqn:qtdefn} is bounded.
This essentially establishes that the effect of a single bad
action is bounded on the long run penalties.

\insertprethmspacing
\begin{lemma}
\label{lem:Bbound}
% Let any one of conditions~\ref{cond:instantaneous}-\ref{cond:moreisbetter}
% be true, and $B$ be as given in Theorem~\ref{thm:finiteactions}.
Let $B$ be as given in Theorem~\ref{thm:finiteactions} for any of
conditions~\ref{cond:instantaneous}-\ref{cond:moreisbetter}.
Then, $\;\sup \qt - \inf \qt \leq B$.
% Then,\\ $\sup \qt - \inf \qt \leq B$.
\begin{proof}
In this proof, $(x,y), (x',y')\in\Xcal\times\Ycal$ will be two pairs of
action-observations.
Denote the action-observations pairs when following $\gopolicy$ after $(x,y)$
by $\Htn$, i.e. $\Htn$ starts with $(x, y)$ and has length $n-t+1$.
Similarly define $\Hptn$ for $(x',y')$. Then
$\qt(x,y) - \qt(x',y') = \EEtt{Y,t+1:n}[r_t]$, where,
\begin{align*}
r_t &= \sumpenl(\thetatrue, \datatmo\concat\Htn)
                  - \sumpenl(\thetatrue, \datatmo\concat\Hptn)
\\
% &= \sumpenl(\thetatrue, \datatmo\concat\{(x,y)\}\concat\Htpon)
%                   - \sumpenl(\thetatrue, \datatmo\concat\{(x',y')\}\concat\Hptpon) \\
&= \sum_{j=t}^n \Big(\penl(\thetatrue, \datatmo\concat\Htj)
                  - \penl(\thetatrue, \datatmo\concat\Hptj) \Big)
% &\qt(x,y) - \qt(x',y') =
% \EEtt{Y,t+1:n}\Big[\sumpenl(\thetatrue, \datatmo\concat\Htn)
%                   - \sumpenl(\thetatrue, \datatmo\concat\Hptn)\Big]
% \\
% &\hspace{0.4in}
% = \EEtt{Y,t+1:n}\Big[\sumpenl(\thetatrue, \datatmo\concat\{(x,y)\}\concat\Htpon)
%                   - \sumpenl(\thetatrue, \datatmo\concat\{(x',y')\}\concat\Hptpon)\Big].
\end{align*}
Here $\sumpenl$ is as defined in~\eqref{eqn:sumpenldefn}.
We will now prove $\qt(x,y) - \qt(x',y') \leq B$ separately for each condition.
%  using one of the
% expressions above for $r_t$.

% \textbf{Condition~\ref{cond:instantaneous}:}
% Under this condition, the penalty
% since $\gopolicy$ knows $\thetatrue$
% \begin{align*}
% r_t &= 
% \end{align*}

\textbf{Condition~\ref{cond:instantaneous}:}
Under this setting, 
$\gopolicy$ which knows $\thetatrue$, will always pick the single best action
which maximises the expected reward.
Hence $\EE_{Y,t+1:n}[r_t] = \penl(\thetatrue, (x,y)) -  \penl(\thetatrue, (x',y'))
\leq 1 = B$.

\textbf{Condition~\ref{cond:recoverability}:}
Denote $\epsilon_j = \penl(\thetatrue, \datatmo\concat\Htj)
- \penl(\thetatrue, \datatmo\concat\Hptj)$.
$\epsilon_j$ is a random quantity for $j\geq t+1$ as it depends on the observations.
We have $r_t = \sum_{j=t}^n \epsilon_j$.
Observe that, at time step $j$, $\gopolicy$ chooses the action to maximise
$\EEtt{\Yx}[\penl(\thetatrue,\datatmo\concat\Htj\concat\{(x,\Yx)\}]$
when starting with $(x,y)$, and 
$\EEtt{\Yx}[\penl(\thetatrue,\datatmo\concat\Hptj\concat\{(x,\Yx)\}]$
when starting with $(x',y')$.
Hence, condition~\ref{cond:recoverability} implies that,
$\EE_{\Ytt{j+1}}[\epsilon_{j+1}] \leq \alpha \epsilon_j$.
% An inductive argument leads to the concl
An inductive argument leads us to,
$\EE_{\Ytt{t+1},\dots,\Ytt{j}}[\epsilon_j] \leq \alpha^{j-t}\epsilon_t$.
However, since $\penl$ maps to $[0,1]$, $\epsilon_t \leq 1$.
Hence $\EEtt{Y,t+1:n}[r_t] \leq \sum_j\alpha^{j-t}\epsilon_t \leq 1/(1-\alpha)=B$.

\textbf{Condition~\ref{cond:moreisbetter}:}
For the purposes of this analysis, we will allow a decision maker to take
no action at time $t-1$ and denote this by $\emptyset$,
i.e. $\datatmo\concat\emptyset\concat\Ftpon$ means the action observation pairs were
$\datatmo$ from time $1$ to $t-1$, then there was no action at time $t$ and then
from time $t+1$ to $n$, the action observation pairs were $\Ftpon$.
In doing so, the decision maker incurs a penalty of $\penl(\thetatrue,\datatmo)$
at step $t+1$.
% In doing so, the decision maker incurs a (maximum) penalty of $1$ at step $t+1$.
% \toworkon{the penalty can also be $\penl(\thetatrue,\datat)$}.
% \toworkon{the penalty can also be $1$}.
Correspondingly, we have,
\begin{align*}
\sumpenl(\thetatrue,\datatmo\concat\emptyset\concat\Ftptn)
 = \sum_{j=1}^{t-1}\penl(\thetatrue,\dataj) + \penl(\thetatrue,\datatmo)
  + \sum_{j=t+2}^n\penl(\thetatrue,\datatmo\concat\Fttnn{t+1}{j}).
\end{align*}
Adding and subtracting $
\sumpenl(\thetatrue, \datatmo\concat\emptyset\concat\Hptnmo)\big)
$ to $r_t$ we have,
% Writing
\begin{align*}
r_t =\;&
\big(\sumpenl(\thetatrue, \datatmo\concat\Htn) -
\sumpenl(\thetatrue, \datatmo\concat\emptyset\concat\Hptnmo)\big)
\numberthis\label{eqn:rtsumtwo}
\;+ \\
&
\big(
\sumpenl(\thetatrue, \datatmo\concat\emptyset\concat\Hptnmo) -
\sumpenl(\thetatrue, \datatmo\concat\Hptn)
\big).
\end{align*}

The second term above can be bounded by $1$ since $\lambda$ maps to $[0,1]$.
\begin{align*}
&\sumpenl(\thetatrue, \datatmo\concat\emptyset\concat\Hptnmo) - 
\sumpenl(\thetatrue, \datatmo\concat\Hptn)
\numberthis\label{eqn:rtone}
\\
&\hspace{0.3in} =
\penl(\thetatrue,\datatmo) + \sum_{j=t+1}^{n-1}\penl(\thetatrue,\datatmo\concat\Hptj)
                           - \sum_{j=t+1}^{n}\penl(\thetatrue,\datatmo\concat\Hptj) \\
&\hspace{0.3in} =
 \penl(\thetatrue,\datatmo) - \penl(\thetatrue, \datatmo\concat\Hptn) \leq 1.
\end{align*}
For the first term, we have,
\begin{align*}
% \EEtmoY\big[
&\big(\sumpenl(\thetatrue, \datatmo\concat\Htn) -
\sumpenl(\datatmo\concat\emptyset\concat\Hptnmo)\big)
\numberthis\label{eqn:rttwo}
\\
&\hspace{0.05in}=
  \big(\penl(\thetatrue, \datatmo\concat\{(x,y)\}) - \penl(\thetatrue, \datatmo)\big)
  \;+\;
% \\
% &\hspace{0.5in}
  \sum_{j=t+1}^n\big(\penl(\thetatrue, \datat\concat\Htj) -
                \penl(\thetatrue, \datat\concat\Hptjmo)\big).
\end{align*}
Recall that
the actions in $\Htj$ are chosen to maximise the expected future rewards.
By condition~\ref{cond:moreisbetter} and since
$\datatmo\cup\{(x,y)\}\supset\datatmo$, each of the 
$n-t$ terms in the RHS summation is less than or equal to zero in expectation
over the observations.
Since $
\penl(\thetatrue, \datatmo\concat\{(x,y)\}) -  \penl(\thetatrue, \datatmo) \leq 1$,
the above term is at most $1$ in expectation over $\EEtt{Y,t+1:n}$.
Combining this with~\eqref{eqn:rtone} gives us
$\EEtt{Y,t+1:n}[r_t] \leq 2 = B$.
% Hence, the above therm is at

\textbf{Condition~\ref{cond:monotonicity}:}
The proof here follows similar to Condition~\ref{cond:moreisbetter},
where we will decompose $r_t$ as the sum of two terms in~\eqref{eqn:rtsumtwo}.
The second term is bounded above by $1$ as in~\eqref{eqn:rtone}.
For the first term in~\eqref{eqn:rttwo},
by the first assumption in condition~\ref{cond:monotonicity},
the first difference in the RHS is non-positive since more data can only
decrease the penalty.
By the second assumption, each of the terms in the summation is also non-positive
since $\Htn$ starts with a lower penalty than $\Hptn$.
\end{proof}

\end{lemma}

\insertprethmspacing

We are now ready to prove theorem~\ref{thm:finiteactions}.

\textbf{\emph{Proof of Theorem~\ref{thm:finiteactions}:}}
First, using the first result of Lemma~\ref{lem:russolemmas} to have,
\begingroup
\allowdisplaybreaks
\begin{align*}
&\EEtmo[\qt(\Xt,\YXt) - \qt(\Xpt,\YXpt)]^2
\\ &\hspace{0.2in}=
\bigg(\sum_{x\in\Xcal}\Ptildetmo(x)
\big(\EEtmo[\qt(x,\Yx)] - \EEtmo[\qt(x,\Yx)|\Xpt=x]\big)
\bigg)^2
\\ &\hspace{0.2in}\leq
|\Xcal| \sum_{x\in\Xcal}
\Ptildetmo(x)^2\big(\EEtmo[\qt(x,\Yx)] - \EEtmo[\qt(x,\Yx)|\Xpt=x]\big)^2
\\ &\hspace{0.2in}\leq
|\Xcal| \sum_{x_1,x_2\in\Xcal}
\Ptildetmo(x_1)\Ptildetmo(x_2)
\big(\EEtmo[\qt(x_1,\Yxone)] - \EEtmo[\qt(x_1,\Yxone)|\Xpt=x_2]\big)^2
\\ &\hspace{0.2in}\leq
\frac{|\Xcal|B^2}{2} \sum_{x_1,x_2\in\Xcal}
\Ptildetmo(x_1)\Ptildetmo(x_2)
\KL(\PPtmo(\Yxone|\Xpt=x_2)\| \PPtmo(x_1))
\\ &\hspace{0.2in}=\frac{1}{2}
|\Xcal|B^2 \MItmo(\Xpt;(\Xt, \YXt))
\,\leq\,
\frac{1}{2}
|\Xcal|B^2 \MItmo(\thetatrue;(\Xt, \YXt))
\end{align*}
\endgroup
Here, the second step uses the Cauchy-Schwarz inequality and
the third step uses the fact that the previous line can be viewed as the
diagonal terms in a sum over $x_1,x_2$.
The fourth step uses a version of Pinsker's inequality given in
Lemma~\ref{lem:pinsker} of Appendix~\ref{app:ancillary}
and the fifth step uses the second result of Lemma~\ref{lem:russolemmas}.
The last step uses Lemma~\ref{lem:misuperset} and the fact that
$\Xpt$ is a deterministic function of $\thetatrue$ given $\datatmo$.
Now, using~\eqref{eqn:lossqt} and the Cauchy-Schwarz inequality we have,
\begin{align*}
\EE[\loss(\thetatrue,\pspolicy) - \loss(\thetatrue,\gopolicy)]^2
&\leq n \sum_{t=1}^n
\frac{1}{2}
|\Xcal|B^2 \MItmo(\thetatrue;(\Xt, \YXt))
=
\frac{1}{2}
|\Xcal|B^2 \MI(\thetatrue;\datan)
\end{align*}
Here the last step uses the chain rule of mutual information in the following form,
\begin{align*}
\sum_t\MItmo(\thetatrue;(\Xt,\YXt)) 
= \sum_t\MI(\thetatrue;(\Xt,\YXt)|\{(\Xj,\YXj)\}_{j=1}^{t-1}) 
= \MI(\thetatrue; \{(\Xj,\YXj)\}_{j=1}^{n}).
\end{align*}
The claim follows from the observation,
$\MI(\thetatrue; \datan)\leq \IGn$.
\hfill
\qedsymbol

\toworkon{
Simple regret with submodular functions.
}


==> archive/regret_apr_28.tex <==

\section{Notes on the Regret for Bayesian DoE}

We will first look at the cumulative regret $\crn$~\eqref{eqn:regretDefn}, which can
be decomposed as follows.
\begin{align*}
\crn &=
\underbrace{ \sumoton\penlt(\thetatrue,\grdatat) - \sumoton\penlt(\thetatrue,\ordatat)}_{
  \cronen}
\;+\; 
\underbrace{ \sumoton\penlt(\thetatrue,\iodatat) - \sumoton\penlt(\thetatrue,\grdatat)}_{
  \crtwon}
\label{eqn:crdecomp}\numberthis
\\
&\quad
\;+\; 
\underbrace{ \sumoton\penlt(\thetatrue,\datat) - \sumoton\penlt(\thetatrue,\iodatat)}_{
  \crthrn}
\end{align*}

Here $\grdatat$ is data chosen by an oracle which knows $\thetatrue$ which adopts
an adaptive greedy strategy -- i.e it executes Algorithm~\ref{alg:bdoe} 
but skips line~\ref{step:sampletheta} and 
in step~\ref{step:choosext} uses $\thetatrue$ instead of a sampled $\theta$ value.
Further, step~\ref{step:initdata} is replaced with $\grdatatt{0}\leftarrow\emptyset$ and
step~\ref{step:adddata} with $\grdatat\leftarrow\grdatatmo\cup\{(\Xt,\Yt)\}$.
Therefore $\cronen$ is the difference between a greedy strategy which knows the
true parameter and the oracle which finds the optimal set at each time step.

Similarly,
$\iodatat$ is an oracle, which, at each time step $t$, uses $\thetatrue$ in
step~\ref{step:choosext} instead of the sampled $\theta$ to select the next action
$\Xpt$, and sets $\iodatat\leftarrow\datatmo\cup \{(\Xpt,\YXpt)\}$.
That is, $\iodatat$ is the same as $\datat$ except for the last action-observation pair.
% by \bdoe, but instead of using a sample $\theta$ from 
Hence, $\crtwon$ is the difference between the greedy strategy which knows the true
parameter and $\iodatat$.
Finally, $\crthrn$ is the sum of differences when $\thetatrue$ is revealed to us versus
when we use the value sampled from the posterior.


\toworkon{I am hoping we could bound $\cronen$ using submodularity, and
$\crtwon$ using Aggrevate.
$\crtwon$ might be the trickiest especially in the cumulative regret setting.}

We will first bound $\crthrn$.
Most ideas here are taken from~\citet{russo2016thompson}.

We will define two quantities which we will need for our purpose.
The first is the information ratio $\IRn$ and second is the maximum information gain
$\IGn$.
\begin{align*}
\IRt &= \frac{\EEtmo[\penlt(\thetatrue,\datat) - \penlt(\thetatrue,\iodatat)]^2}{%
 \Itmo(\thetatrue; (\Xt, \YXt)) }
\numberthis\label{eqn:infratio}
 \\
\IGt &= \max_{\datat\subset\Dcalt} I(\thetatrue; \datat)
\numberthis\label{eqn:mig}
\end{align*}

\insertprethmspacing
\begin{theorem}
\label{prop:baseprop}
For all $n\geq 0$, if $\IRt\leq\IRbar$ for all $t\leq n$, then,
\emph{
\[
\EE[\crthrn] \leq
  \sqrt{n\IRn\IGn}
\]
}
\begin{proof}
First using the quantities above and the Cauchy-Schwarz inequality we have,
\begin{align*}
\EE[\crthrn] \;&\leq\;
\EE\sumoton\EEtmo[\penlt(\thetatrue,\datat) - \penlt(\thetatrue,\iodatat)]
% \\
\leq\; \sqrt{\IRbar}\left(\EE\sumoton\sqrt{\It(\thetatrue;(\Xt,\YXt))}\right)
\\
&\leq \sqrt{n\IRbar\sumoton\EE[\Itmo(\thetatrue;(\Xt,\YXt))]}.
\end{align*}
We conclude the proof with the following calculation which uses the chain rule for
mutual information.
\begin{align*}
\sumoton \EE\Itmo(\thetatrue; (\Xt,\YXt)) =
\sumoton I(\thetatrue; (\Xt, \YXt) | \datatmo) = I(\thetatrue; \datan) \leq \IGn.
\end{align*}
\end{proof}
\end{theorem}

\toworkon{I can bound $\IRn$ using techniques in~\citet{russo2016thompson} and
$\IGn$ using techniques in~\citet{srinivas10gpbandits}.}



==> archive/regret_may_14.tex <==

\section{Notes on the Regret for Bayesian DoE}
\label{sec:regret}


Following the plurality of the on-line learning literature,
our goal is to collect data $\dataseqn$
so as to achieve a small cumulative sum of
penalties after $n$ steps as defined below,
% $\dataseqn$, we wish to minimise the cumulative penalties as defined below,
\begin{align*}
\sumpenl(\thetatrue, \dataseqn) = \sum_{t=1}^n\penl(\thetatrue, \dataseqt)
= \sum_{t=1}^n\penl(\thetatrue, \{(\Xj,\Yj)\}_{j=1}^t).
\numberthis
\label{eqn:sumpenldefn}
\end{align*}
The loss $\lossn(\thetatrue,\policy)$ of a policy $\pi$ after $n$ evaluations is the
expected
loss of cumulative penalties $\lossn(\thetatrue,\policy) =
\EE[\sumpenl(\thetatrue,\dataseqn)]$
where $\dataseqn$ is collected by following $\policy$.

Our goal in this section is to analyse settings where a myopic strategy would work well.
To that end, 
let $\gopolicy$ be the policy that behaves in a myopic manner, but knows the true
value of $\thetatrue$.
Let $\godatat$ to be the data collected by this policy  in $t$ steps.
That is $\gopolicy$ follows Algorithm~\ref{alg:bdoe} 
but skips line~\ref{step:sampletheta} and 
in step~\ref{step:choosext} uses $\thetatrue$ instead of a sampled $\theta$ value.
Further, step~\ref{step:initdata} is replaced with $\godatatt{0}\leftarrow\emptyset$ and
step~\ref{step:adddata} with $\godatat\leftarrow\godatatmo\concat\{(\Xt,\Yt)\}$.
We will show that the policy $\pspolicy$ in Algorithm~\ref{alg:bdoe},
is competitive with $\gopolicy$.
That is, if we define the regret of a policy $\policy$ after $n$ evaluations as,
\begin{align*}
R(\thetatrue, \policy) &=
  \loss(\thetatrue, \policy) - \loss(\thetatrue, \gopolicy)
  = \EE\sum_{t=1}^n \penl(\thetatrue, \datat)\, -\, 
        \EE\sum_{t=1}^n \penl(\thetatrue, \godatat), %\\
\label{eqn:regretDefn}\numberthis
% \frn &= \penln(\thetatrue, \datan)\, -\, \penln(\thetatrue, \ordatan)
\end{align*}
then $R(\thetatrue,n,\pspolicy)$ is sub-linear in $n$.
The expectation above is over the observations and the randomness of our policy $\pi$.
The regret in~\eqref{eqn:regretDefn} is itself a random quantity since $\thetatrue$
is random, so we will consider the
Bayesian regret $\EEtt{\thetatrue\sim\pthetazero}[R(\thetatrue,n,\policy)]$,
taking expectation
over the prior $\pthetazero$.

\toworkon{Why this is difficult without assumptions. Refer to RL literature.}

% which, essentially imply that taking an action does not hurt

We will argue that under a variety of conditions on the penalty function,
the above algorithm will achieve sub-linear regret.
The first such condition states that the penalty function can only depend on a
finite number of action-observations at any time step.

% \insertprethmspacing
% \begin{condition}[Finite dependence on Actions]
% \label{cond:instantaneous}
% Let $K\in\NN_+$ and 
% let $\sigma:\NN \rightarrow 2^\NN$ be a deterministic function such that
% $t-K\leq s \leq t$ for all $s\in\sigma(t)$ and $|\sigma(t)| \leq K$.
% For a data sequence $\datat$, let $\datatt{t,\sigma(t)} = \{(\Xj,\YXj): j\in\sigma(t)\}$.
% Than, at any given time step, $\penl$ depends only on the actions and observations
% taken at the time steps in $\sigma(t)$;
% i.e. $\penl(\thetatrue,\datat) = \penl(\thetatrue,\datatt{t, \sigma(t)})$
% \end{condition}

\insertprethmspacing
\begin{condition}[Episodic Penalties]
% \label{cond:instantaneous}
\label{cond:instantaneous}
The infinite sequence can be divided into ``episodes'' of length $H$ where
episode $j$ consists of time steps $(j-1)H + 1$ to $jH$.
The penalty at a given time step depends only on the action and observation of the current
episode. That is, 
$\penl(\thetatrue,\datat) = \penl(\thetatrue,\{(\Xj, \YXj)\}_{j=t'}^t)$
and $t'$ is the start time of the current episode.
\end{condition}

% A simple example where Assumption~\ref{cond:instantaneous} holds is a moving average
% bandit where the reward at the current time step is the average of the last
% $K$ rewards.
The next condition under which we can achieve sub-linear regret is recoverability.

\insertprethmspacing
\begin{condition}[Recoverability]
\label{cond:recoverability}
There exists $\alpha<1$ such that for data sequences $D_1, D_2$ with
$\penl(\thetatrue, D_1) \leq \penl(\thetatrue, D_2) + \epsilon$,
we have,
\[
\max_{x\in\Xcal} \EEtt{\Yx}[\penl(\thetatrue, D_1\concat (x,\Yx))]
\leq \max_{x\in\Xcal} \EEtt{\Yx}[\penl(\thetatrue, D_2\concat (x,\Yx))] +
\alpha\epsilon.
\]
\end{condition}
\toworkon{Only need this for length one deltas.}

Assume that we have two data sequences $D_1$ and $D_2$ where $D_1$ is worse than $D_2$
by up to $\epsilon$.
Condition~\ref{cond:recoverability} states that the best point we can choose with the
``bad'' dataset $D_1$ improves on this slack by a factor $\alpha$ in comparison to the
best point choosable with $D_2$.
Intuitively, this states that even if we were unfortunate to have had bad observations
and hence large penalty $\penl$, there is opportunity to
recover and eventually start performing well.
\toworkon{
Link this to mixing time in RL.
}

% The next two conditions capture properties that are common in data accumulation tasks,
% such as active learning,
% where a greedy policy 
% The next two conditions state that the myopic policy which knows $\thetatrue$, i.e.
% $\gopolicy$, behaves reasonably.
% In common data accumulation tasks, one expects a rational policy
% The following two conditions
%  is when the penalty function satisfies some monotonicity conditions.

The next two conditions assume some regularity conditions on $\penl$ when collecting
data according to $\gopolicy$.
Accordingly, we will show that when a myopic policy which knows $\thetatrue$
can behave reasonably, so can posterior sampling. 

\insertprethmspacing
\begin{condition}[Monotonicity]
  For all $x\in\Xcal$,
  $\penl(\thetatrue, D\concat\{(x,\Yx)\}) \,\leq\, \penl(\thetatrue, D)$.
  Further,
  let $D_1,D_2\in\Dcal$ be such that $\penl(\thetatrue, D_1) \leq \penl(\thetatrue, D_2)$.
  Let $H_1,H_2$ be equal length ($|H_1| = |H_2|$) data sequences
  collected by $\gopolicy$ when executed from $D_1$ and $D_2$ respectively.
  Let $\Ytt{H_i}\in\Ycal^{|H_1|}$ be the observations when taking the actions in $H_i$.
  Then $\EEtt{\Ytt{H_1}}[\penl(\thetatrue, D_1\concat H_1)] \leq
      \EEtt{\Ytt{H_2}}[\penl(\thetatrue, D_2\concat H_2)]$.
\label{cond:monotonicity}
\end{condition}

Condition~\ref{cond:monotonicity}
captures two notions of monotonicity on $\penl$.
The first, is that adding more data always shrinks the penalty function.
The second, is that when following $\gopolicy$ from a better dataset (less penalty),
the penalty accumulated is no worse than if we had started with a bad dataset.
The next condition captures a similar notion of reasonable behaviour for $\thetatrue$
which says that $\gopolicy$ can always
make better decisions when it has more data.

\insertprethmspacing
\begin{condition}[More data is better]
  Let $D_1,D_2\in\Dcal$ be such that $D_1 \supset D_2$.
  Let $H_1,H_2$ be equal length ($|H_1| = |H_2|$) data sequences
  collected by $\gopolicy$ when executed from $D_1$ and $D_2$ respectively.
  Let $\Ytt{H_i}\in\Ycal^{|H_1|}$ be the observations when taking the actions in $H_i$.
  Then $\EEtt{\Ytt{H_1}}[\penl(\thetatrue, D_1\concat H_1)] \leq
      \EEtt{\Ytt{H_2}}[\penl(\thetatrue, D_2\concat H_2)]$.
% \label{cond:monotonicity}
\label{cond:moreisbetter}
\end{condition}



Note that the conditions~\ref{cond:recoverability},%
~\ref{cond:monotonicity} and~\ref{cond:moreisbetter}
are stated with respect to the true parameter $\thetatrue$;
i.e. that good actions \emph{can} be chosen so as to achieve certain conditions.
Hence, they are essentially conditions on the properties of the penalty function.
While a policy which knows $\thetatrue$, such as $\gopolicy$, which can compute the exact 
expected value of future penalties, can always correctly choose such actions,
this may not be the case for a policy such as $\pspolicy$ which does not know
$\thetatrue$.
 
To state our main theorem, we introduce the maximum information gain (MIG)
$\IGn$.
\begin{align*}
% \IRt &= \frac{\EEtmo[\penlt(\thetatrue,\datat) - \penlt(\thetatrue,\iodatat)]^2}{%
%  \Itmo(\thetatrue; (\Xt, \YXt)) }
% \numberthis\label{eqn:infratio}
%  \\
\IGn &= \max_{\datan\subset\Dcaln} I(\thetatrue; \datan)
\numberthis\label{eqn:mig}
\end{align*}
Here $I$ is the Shannon mutual information.
$\IGn$ measures the maximum information a set of $n$ action-observation pairs can
tell us about the true parameter $\thetatrue$.
% The MIG is a natural quantity to capture the statistical complexity of a discriminative
% model $\PP(Y|X,\thetatrue)$  in the Bayesian paradigm.
The quantity was first introduced for Gaussian processes
by~\citet{srinivas10gpbandits}, and has been popularly
% used in regret bounds in various Bayesian adaptive data analysis settings such as
used to measure the statistical complexity of various Bayesian adaptive data analysis
settings such as Bayesian optimisation~\citep{srinivas10gpbandits},
active learning~\citep{ma2015active},
and level set estimation~\citep{gotovos2013active}.
Below, we list some examples of common models which demonstrate that
$\IGn$ is sublinear in $n$.

\insertprethmspacing
% \begin{example}[Bounds on the MIG for common models~\citep{srinivas10gpbandits}]
\begin{example}Bounds on the MIG for common models~\citep{srinivas10gpbandits}.
\begin{enumerate}
\item \textbf{Linear models:}
Let $\Xcal\subset\RR^d$, $\theta\in\RR^d$,
 and $\Yx|x,\theta \sim\Ncal(\theta^\top x, \eta^2)$.
For a multi-variate Gaussian prior on $\thetatrue$, $\IGn\in\bigO(d\log(n))$.
\item \textbf{Gaussian process:}
Let $\Xcal\subset\RR^d$.
Assume a Gaussian process prior
$\thetatrue\sim\GP(\mu,\kernel)$,
and Gaussian observations $\Yx|x,\theta \sim\Ncal(\theta(x), \eta^2)$.
Here $\mu:\Xcal\rightarrow\RR$ is the prior mean of the GP and
$\kernel:\Xcal^2\rightarrow\RR$ is the covariance kernel.
When $\kernel$ is an RBF kernel, $\IGn\in\bigO(\log(n)^{d+1})$.
When $\kernel$ is a mat\'ern kernel, $\IGn\in\bigO(n^p\log(n))$ for some $p<1$.
\end{enumerate}
\end{example}

% In general, one expects the regret in an interactive model to depend on the complexity
% of the model and 
% While the MIG is not known
% The MIG provides us a way to abstract out the statistical complexity of a model.
We are now ready to state our main theorem
under \emph{any} one of the above conditions we have the following theorem.

\insertprethmspacing
\begin{theorem}
\label{thm:finiteactions} 
Assume \textbf{any one} of conditions~\ref{cond:instantaneous}-\ref{cond:moreisbetter}
hold.
Let $B=1$ under conditions~\ref{cond:instantaneous} and~\ref{cond:monotonicity},
$B=1/(1-\alpha)$ under condition~\ref{cond:recoverability},
% $B=1$ under condition~\ref{cond:monotonicity},
and $B=2$ under condition~\ref{cond:moreisbetter}.
Then if $\Xcal$ is finite,
\[
\EE[\lossn(\thetatrue,\pspolicy) - \lossn(\thetatrue, \gopolicy)]
\leq B\sqrt{\frac{1}{2}n|\Xcal|\IGn}
\]
\end{theorem}
\toworkon{Comment on $\IGn$ and $|\Xcal|$ dependence. Why do both appear?}





==> archive/regret_may_3.tex <==

\section{Notes on the Regret for Bayesian DoE}

Let $\gopolicy$ be the policy that behaves in a myopic manner, but knows the true
value of $\thetatrue$.
Let $\godatat$ to be the data collected by this policy  in $t$ steps.
That is $\gopolicy$ follows Algorithm~\ref{alg:bdoe} 
but skips line~\ref{step:sampletheta} and 
in step~\ref{step:choosext} uses $\thetatrue$ instead of a sampled $\theta$ value.
Further, step~\ref{step:initdata} is replaced with $\godatatt{0}\leftarrow\emptyset$ and
step~\ref{step:adddata} with $\godatat\leftarrow\godatatmo\cup\{(\Xt,\Yt)\}$.
We will show that the policy $\policy$ in Algorithm~\ref{alg:bdoe},
is competitive with $\gopolicy$.
That is, if we define the regret
\begin{align*}
\creg(\thetatrue, n) &=
  \loss(\thetatrue, \pi) - \loss(\thetatrue, \gopolicy)
  = \EE\sum_{t=1}^n \penl(\thetatrue, \datat)\, -\, 
        \EE\sum_{t=1}^n \penl(\thetatrue, \ordatat), %\\
\label{eqn:regretDefn}\numberthis
% \frn &= \penln(\thetatrue, \datan)\, -\, \penln(\thetatrue, \ordatan)
\end{align*}
then $\creg$ is sublinear in $n$.
The expectation above is over the observations and the randomness of our policy $\pi$.
The regret in~\eqref{eqn:regretDefn} is itself a random quantity since $\thetatrue$
is random, so we will consider the
Bayesian regret $\bcrn = \EE[\crn]$, where the expectation
is over the prior $\pthetazero$.

\toworkon{Why this is difficult without assumptions. Refer to RL literature.}

We will need the following two monotonicity conditions on the penalty function.
% which, essentially imply that taking an action does not hurt

\insertprethmspacing
\begin{assumption}[Monotonicit of $\penl$]
\label{asm:penlregularity}
Let $\penl:\Theta\times\Dcal\rightarrow[0,1]$ be the penalty function. Let
$D\in\Dcal$ be an already observed data sequence of action-observation pairs.
Let $V\subset\Xcal$ be a finite subset of actions,
$Y_V=\{\YX: X\in V\}$ be the (yet unobserved) results of the experiments at $V$,
and $\widetilde{V} = \{(X, \YX): X\in V\}$ be the action-observation pairs at $V$.
Further, let $P_1,P_2 \subset\Xcal$ be finite subsets of $\Xcal$,
and similarly define $\Ytt{P_1},\Ytt{P_2},\widetilde{P}_1, \widetilde{P}_2$.
\begin{enumerate}
\item 
  For all $V\subset\Xcal$,
  $\quad\EE_{\Ytt{V}}[\penl(\theta, D\cup\widetilde{V})] \,\leq\, \penl(\theta, D)$.
\item
%   For $\theta\in\Theta$ and $D\in\Dcal$, 
  Let $P_1,P_2$ be such that
  $\;\EE_{\Ytt{P_1}}[\penl(\theta, D\cup\widetilde{P}_1)] \,\leq\,
    \EE_{\Ytt{P_2}}[\penl(\theta, D\cup\widetilde{P}_2)]$.
  Then, for all $V\subset\Xcal$,
  $\;\EE_{\Ytt{P_1}, \Ytt{V}}[\penl(\theta, D\cup\widetilde{P}_1\cup\widetilde{V})]
    \,\leq\,
    \EE_{\Ytt{P_2}, \Ytt{V}}[\penl(\theta, D\cup\widetilde{P}_2\cup\widetilde{V})]$.
\end{enumerate}
\end{assumption}
\toworkon{check quantifiers!}

To motivate these assumptions, assume that we have already collected a data
sequence $D$.
The first condition says that taking additional actions, i.e. additional data,
 does not increase the penalty.
For example, in active learning settings, while choosing a new data point to be labelled
may not significantly improve our estimate, it does not worsen it either.
Since the observations are random, so is the penalty after taking the actions in $V$;
we require monotonicity to hold in expectation, which reflects practical settings
and is weaker than
assuming it to be true for all $Y\in\Ycal$.
For the second condition, assume that we have already queried at $D$ and have the
option of choosing either ${P}_1$ or ${P}_2$ for free,
but ${P}_1$ is expected to do better in expectation.
Then, the addition of a new data sequence $V$, does not improve the latter setting 
better than the former.
Therefore, choosing the set that does better now will not hurt us down the line.
We finally note that we will need both conditions of Assumption~\ref{asm:penlregularity}
to hold only when $|V| = 1$.

\toworkon{Spiel on why these assumptions pave way to a myopic strategy.
Refer to submodular maximization which makes monotonicity assumptions on $f$.}

\subsection*{Proofs}

\textbf{Notation and Set up:}
We will introduce some notation before we proceed.
Let $\datat\in\Dcalt$ be a set of $t$ action-observation pairs.
Then, $\Qpi(\datat,x)$ will denote the expected total penalty when we take action
$x$ and then execute policy $\policy$ for the remaining $n-t-1$ steps.
That is,
\begin{align*}
\numberthis\label{eqn:Qdefn}
&\Qpi(\datat, x) = \EE\big[\sumpenl(\thetatrue, \datat\cup\{(x, \Yx)\}\cup\Ftptn) \big] \\
&\hspace{0.05in}
= \sum_{j=1}^t\penl(\thetatrue, \dataj) +
  \EE_{\Yx, \Ftptn}\bigg[\penl(\thetatrue, \dataj\cup\{(x,\Yx)\})
%   &\hspace{0.3in}
  + \sum_{j=t+2}^n \penl(\thetatrue, \dataj\cup\{(x,\Yx)\}\cup
      \Fttnn{t+2}{j} ) \bigg]
\end{align*}
Here, the action-observation pairs collected by $\policy$
from steps $t+2$ to $n$ are $\Ftptn$.
Note that $\Qpi$ is a function of the true parameter $\thetatrue$.
Moreover, we will denote the distribution of $\datat$ when following a policy $\pi$
for the first $t$ steps to be $\dttpp{t}{\pi}$.
With this notation, we have,
\begin{align*}
J(\thetatrue,\policy) = \EE_{\datat\sim\dttpp{t}{\policy}}
\big[\EE_{X\sim\policy(\datat)}[\Qpp{\policy}(\datat, X)]\big].
\numberthis \label{eqn:lossQ}
\end{align*}
Finally, for the purposes of the analysis, we will allow a decision maker to take
no action at any given time step $t$ and denote this by $\emptyset$,
i.e. $\datat\cup\emptyset\cup\Ftptn$ means the action observation pairs were
$\datat$ from time $1$ to $t$, then there was no action at time $t+1$ and then
from time $t+2$ to $n$, the action observation pairs were $\Ftptn$.
In doing so, the decision maker incurs a penalty of $\penl(\thetatrue,\datat)$
at step $t+1$.
% In doing so, the decision maker incurs a (maximum) penalty of $1$ at step $t+1$.
% \toworkon{the penalty can also be $\penl(\thetatrue,\datat)$}.
\toworkon{the penalty can also be $1$}.
Correspondingly, we have,
\begin{align*}
\sumpenl(\thetatrue,\datat\cup\emptyset\cup\Ftptn)
 = \sum_{j=1}^t\penl(\thetatrue,\dataj) + \penl(\thetatrue,\datat)
  + \sum_{j=t+2}^n\penl(\thetatrue,\datat\cup\Fttnn{t+2}{j})
\end{align*}

We will need the following Lemma for our analysis.
The proof is adapted from Lemma 4.3 in~\citet{ross2014reinforcement}.

\insertprethmspacing
\begin{lemma}
For any two policies $\policyone,\policytwo$,
\begin{align*}
&J(\thetatrue,\policyone) - J(\thetatrue,\policytwo) = \\
% = \sum_{t=1}^n \EE_{\datatmo \sim \dtmopo, X\sim\policyone(\datatmo)}\left[
%  \Qpt(\datatmo, X) \right]
%  -\EE_{\datatmo \sim \dtmopo, X\sim\policytwo(\datatmo)}\left[
%  \Qpt(\datatmo, X) \right]
&\hspace{0.4in} \sum_{t=1}^n \EE_{\datatmo \sim \dtmopo}\left[
  \EE_{X\sim\policyone(\datatmo)}\left[
 \Qpt(\datatmo, X) \right]
 -\EE_{X\sim\policytwo(\datatmo)}\left[
 \Qpt(\datatmo, X) \right]
  \right]
\end{align*}
\label{lem:valuedecomp}
\begin{proof}
Let $\policy^t$ be the policy that follows $\policyone$ from time step $1$ to $t$, and
then executes policy $\policytwo$ from $t+1$ to $n$.
Hence, by~\eqref{eqn:lossQ}, 
\[J(\thetatrue, \policy^t) 
=\; \EE_{\datatmo\sim\dttpp{t-1}{\policyone}}
\big[\EE_{X\sim\policyone(\datatmo)}[\Qpp{\policytwo}(\datatmo, X)]\big]
=\;
\EE_{\datat\sim\dttpp{t}{\policyone}}
\big[\EE_{X\sim\policytwo(\datat)}[\Qpp{\policytwo}(\datat, X)]\big]
\]
The claim follows from the observation,
$
J(\thetatrue, \policyone) - J(\thetatrue, \policytwo) =
J(\thetatrue, \policy^n) - J(\thetatrue, \policy^0) =
\sum_{t=1}^n J(\thetatrue, \policy^t) - J(\thetatrue, \policy^{t-1}).
$
% &\hspace{0.2in}
% = \sum_{t=1}^n J(\thetatrue, \policy^t) - J(\thetatrue, \policy^{t-1}) \\
\end{proof}
\end{lemma}

\insertprethmspacing
\begin{theorem}[Main Theorem]
\label{thm:mainone}
Here ..
\begin{proof}
We will first use Lemma~\ref{lem:valuedecomp} to express the regret as a sum of
$n$ terms.
For this, 
denote the action chosen by $\policy$ when it has seen data $\datatmo$
as $\Xt$.
%  and that taken by $\gopolicy$ as $\Xpt$. %, i.e. $\Xt\sim\policy(\datatmo)$
% and $\Xpt\sim\gopolicy(\datatmo)$.
Further, denote the action-observations pairs when choosing
$\Xt\sim\policy(\datatmo)$ and then following $\gopolicy$
as $\Htmotn$, i.e. $\Htmotn$ includes $(\Xt, \YXt)$ and has length $n-t+1$.
Similarly,  denote the action chosen by $\gopolicy$ when it has seen data $\datatmo$
as $\Xpt$ and the ensuing $n-t+1$ action-observations pairs when following
$\gopolicy$ as $\Hptmotn$.
By Lemma~\ref{lem:valuedecomp} and equation~\eqref{eqn:Qdefn} we have,
\begin{align*}
\EE_{\thetatrue}[\loss(\thetatrue,\policy) - \loss(\thetatrue,\gopolicy)]
&= \EE \sum_{t=1}^n \EEtmo\Big[
 \underbrace{\Qpp{\gopolicy}(\datatmo,\Xt)
 - \Qpp{\gopolicy}(\datatmo,\Xpt)}_{r_t} \Big] \\
% \underbrace{\Qpp{\gopolicy}(\datatmo,\Xt)
%  - \Qpp{\gopolicy}(\datatmo,\Xpt) }_{r_t}  \Big]
&= \EE \sum_{t=1}^n \EEtmo\Big[
\underbrace{\sumpenl(\datatmo\cup\Htmotn)
 - \sumpenl(\datatmo\cup\Hptmotn)}_{r_t} \Big] \\
\end{align*}
Note that $\EEtmo$, which conditions on $\datatmo$ collected by $\policy$,
encompasses three sources of randomness.
The first is due to the randomness in the problem due to $\thetatrue\sim\pthetazero$,
the second is due to the observations $Y\sim\PP(\cdot|X,\thetatrue)$,
and the third 
is an external source of randomness $U$ used by the decision maker in
step~\ref{step:sampletheta} in Algorithm~\ref{alg:bdoe}.
While the actions $\{\Xt\}_t$ chosen depends on all sources of randomness, these
three sources are themselves independent.
Therefore, we can write $\EEtmo[r_t] = \EEU[\EEtmorho[\EEtmoY[r_t]]]$
where $\EEU$ captures the randomness by the decision maker,
$\EEtmorho$ due to the prior
and
$\EEtmoY$ due to the observations.

We will now argue $\EEtmoY[r_t] \leq 1$.
Adding and subtracting $
\sumpenl(\thetatrue, \datatmo\cup\emptyset\cup\Hptmotnmo)\big)
$ we have,
% Writing
\begin{align*}
r_t =\;&
\big(\sumpenl(\thetatrue, \datatmo\cup\Htmotn)  -
\sumpenl(\thetatrue, \datatmo\cup\emptyset\cup\Hptmotnmo)\big)
\;+ \\
&
\big(
\sumpenl(\thetatrue, \datatmo\cup\emptyset\cup\Hptmotnmo) - 
\sumpenl(\thetatrue, \datatmo\cup\Hptmotn)
\big).
\end{align*}
The second term above can be bounded by $1$ since $\lambda$ maps to $[0,1]$.
\begin{align*}
&\sumpenl(\thetatrue, \datatmo\cup\emptyset\cup\Hptmotnmo) - 
\sumpenl(\thetatrue, \datatmo\cup\Hptmotn) \\
&\hspace{0.3in} =
\penl(\thetatrue,\datatmo) + \sum_{j=t+1}^{n-1}\penl(\thetatrue,\datatmo\cup\Hptmotj)
                           - \sum_{j=t+1}^{n}\penl(\thetatrue,\datatmo\cup\Hptmotj) \\
&\hspace{0.3in} =
 \penl(\thetatrue,\datatmo) - \penl(\thetatrue, \datatmo\cup\Hptmotn) \leq 1.
\end{align*}
For the first term, we similarly have,
\begin{align*}
% \EEtmoY\big[
&\big(\sumpenl(\thetatrue, \datatmo\cup\Htmotn)  -
\sumpenl(\datatmo\cup\emptyset\cup\Hptmotnmo)\big) \\
&\hspace{0.2in}= 
  \big(\penl(\thetatrue, \datatmo\cup\{(\Xt,\YXt)\}) -  \penl(\thetatrue, \datatmo)\big)
  \;+\;
\\
&\hspace{0.5in}
  \sum_{j=t+1}^n\big(\penl(\thetatrue, \datat\cup\Htmotj) -
                \penl(\thetatrue, \datat\cup\Hptmotjmo)\big).
\end{align*}
We will show that each of $n-t+1$ terms in the RHS sum are non-positive in
expectation via an inductive argument.
We use the first term as the base step,
where we have,
$\EEtt{\YXt}[\penl(\thetatrue, \datatmo\cup\{(\Xt,\YXt)\})]
\leq \penl(\thetatrue, \datatmo)$ by the first monotonicity condition
in Assumption~\ref{asm:penlregularity}.
For the inductive step, assume that
$\EEtmoY[\penl(\thetatrue, \datat\cup\Htmotj) -
         \penl(\thetatrue, \datat\cup\Hptmotjmo)] \leq 0$.
Then, by the second monotonicity condition,
$\EEtmoY[\penl(\thetatrue, \datat\cup\Htmotjpo) -
         \penl(\thetatrue, \datat\cup\Hptmotj)] \leq 0$.
% $r_t = \sumpenl(\datatmo\cup\Htmotn) - \sumpenl(\datatmo\cup\Hptmotnmo)
% +
We conclude the proof as follows,
\begin{align*}
\EEtmo[r_t] = \EEU[\EEtmorho[\EEtmoY[r_t]]]
\end{align*}
TBC.
\end{proof}
\end{theorem}

% We will define two quantities which we will need for our purpose.
% The first is the information ratio $\IRn$ and second is the maximum information gain
% $\IGn$.
% \begin{align*}
% \IRt &= \frac{\EEtmo[\penlt(\thetatrue,\datat) - \penlt(\thetatrue,\iodatat)]^2}{%
%  \Itmo(\thetatrue; (\Xt, \YXt)) }
% \numberthis\label{eqn:infratio}
%  \\
% \IGt &= \max_{\datat\subset\Dcalt} I(\thetatrue; \datat)
% \numberthis\label{eqn:mig}
% \end{align*}
% 
% \insertprethmspacing
% \begin{theorem}
% \label{prop:baseprop}
% For all $n\geq 0$, if $\IRt\leq\IRbar$ for all $t\leq n$, then,
% \emph{
% \[
% \EE[\crthrn] \leq
%   \sqrt{n\IRn\IGn}
% \]
% }
% \begin{proof}
% First using the quantities above and the Cauchy-Schwarz inequality we have,
% \begin{align*}
% \EE[\crthrn] \;&\leq\;
% \EE\sumoton\EEtmo[\penlt(\thetatrue,\datat) - \penlt(\thetatrue,\iodatat)]
% % \\
% \leq\; \sqrt{\IRbar}\left(\EE\sumoton\sqrt{\It(\thetatrue;(\Xt,\YXt))}\right)
% \\
% &\leq \sqrt{n\IRbar\sumoton\EE[\Itmo(\thetatrue;(\Xt,\YXt))]}.
% \end{align*}
% We conclude the proof with the following calculation which uses the chain rule for
% mutual information.
% \begin{align*}
% \sumoton \EE\Itmo(\thetatrue; (\Xt,\YXt)) =
% \sumoton I(\thetatrue; (\Xt, \YXt) | \datatmo) = I(\thetatrue; \datan) \leq \IGn.
% \end{align*}
% \end{proof}
% \end{theorem}
% 
% \toworkon{I can bound $\IRn$ using techniques in~\citet{russo2016thompson} and
% $\IGn$ using techniques in~\citet{srinivas10gpbandits}.}

\toworkon{
Simple regret with submodular functions.
}


==> regret_old.tex <==

\section{Theoretical Analysis}
\label{sec:regret}

% We will define two notions of regret, corresponding to the two criteria
% in~\eqref{eqn:penldefn}, after collecting a data sequence
% $\datan$ in $n$ experiments.
The goal of this analysis is to study the conditions under which a myopic policy such as
$\pspolicy$ can perform well, when the penalty is not observed.
We will show that $\pspolicy$ is competitive with two policies that know 
$\thetatrue$ under suitable assumptions on the problem.
The first is $\gopolicy$, described previously, against which
$\pspolicy$ compares favourably on  on both criteria
$\cridx$ and $\fridx$ in~\eqref{eqn:penldefn}.
% For this, we will first introduce two oracle policies that know $\thetatrue$.
% That is, if $\godatat$ to be the data collected by this policy  in $t$ steps.
% That is $\gopolicy$ follows Algorithm~\ref{alg:bdoe}
% but skips line~\ref{step:sampletheta} and
% in step~\ref{step:choosext} uses $\thetatrue$ instead of a sampled $\theta$ value.
% Further, step~\ref{step:initdata} is replaced with $\godatatt{0}\leftarrow\emptyset$ and
% step~\ref{step:adddata} with $\godatat\leftarrow\godatatmo\concat\{(\Xt,\Yt)\}$.
% As we will see,
% $\pspolicy$ is competitive with $\gopolicy$ on both criteria
% $\cridx$ and $\fridx$ in~\eqref{eqn:penldefn} under suitable assumptions.
The second policy $\gopolicy$ behaves in a globally optimal adaptive fashion with respect
to $\thetatrue$ for $n$ evaluations.
That is, if $\uodatam$ is the data collected by $\uopolicy$,
$\EE[\penl(\thetatrue, \uodatan)] = \min_{\datan \in \Dcaln}
\EE[\penl(\thetatrue, \datan)]$. \akshay{This defn doesn't parse since $\datan$ includes the observations!}
Unlike $\gopolicy$, we are unable to exactly specify what $\uopolicy$ is.
% Observe that i
Yet, we will argue that $\pspolicy$ is competitive with $\uopolicy$ on
criteria $\fridx$ in~\eqref{eqn:penldefn}.  A comparison with
$\uopolicy$ on $\cridx$ is meaningless since it might take high
penalty actions in the early stages in order to do well in the long
run.  Hence, $\uopolicy$ might not achieve a good $\sumpenl$ value.
\akshay{Might want to phrase this in a different way. I guess you
  could define a globally optimal policy for the cumulative regret, by
  $\pi^{\star\star}$ is not it, and you don't want people to ask this
  question. Maybe just say ``since in most of our applications we are
  interested in final performance, we focus on that when comparing
  with $\pi^{\star\star}$.}
% We also mention that
% Observe that
% both $\gopolicy$ and $\uopolicy$ are not realisable since they assume access to the
% true parameter $\thetatrue$.

% We begin with the following notion of regret which compares
% a policy $\policy$ against $\gopolicy$ on criteria $\cridx$.
Let
the loss $\lossn(\thetatrue,\policy)$ of a policy $\policy$ after $n$ evaluations be
the expected sum of cumulative penalties for fixed $\thetatrue$,
i.e. $\lossn(\thetatrue,\policy) =
\EE[\sumpenl(\thetatrue,\dataseqn)|\thetatrue,\policy]$.
Here $\dataseqn$ is the data sequence collected when following $\policy$.
For criterion $\cridx$, we define the regret of a policy $\policy$ after $n$ evaluations
with respect to $\gopolicy$ as,
\begin{align*}
% R(\thetatrue, \policy) &=
  \lossn(\thetatrue, \policy) - \lossn(\thetatrue, \gopolicy)
  = \EE[\sumpenl(\thetatrue, \datan)|\thetatrue,\policy] - \EE[\sumpenl(\thetatrue, \godatan)|\thetatrue,\gopolicy].
%   = \EE\sum_{t=1}^n \penl(\thetatrue, \datat)\, -\, 
%         \EE\sum_{t=1}^n \penl(\thetatrue, \godatat). %\\
\label{eqn:regretDefn}\numberthis
% \frn &= \penln(\thetatrue, \datan)\, -\, \penln(\thetatrue, \ordatan)
\end{align*}
The expectations are over
the observations and any randomness in the policies.
This regret is itself a random quantity since $\thetatrue$
is random, so we will consider the
Bayesian regret $\EEtt{\thetatrue\sim\pthetazero}[\lossn(\thetatrue,\policy)
-\lossn(\thetatrue, \gopolicy)]$,
taking expectation over the prior $\pthetazero$.
% then $R(\thetatrue,n,\pspolicy)$ is sub-linear in $n$.
% The expectation above is over the observations and the randomness of our policy $\pi$.
% The regret in~\eqref{eqn:regretDefn} is itself a random quantity since $\thetatrue$
% is random, so we will consider the
% Bayesian regret $\EEtt{\thetatrue\sim\pthetazero}[R(\thetatrue,n,\policy)]$,
% taking expectation
% over the prior $\pthetazero$.

% \akshay{I suggest stating this as a proposition.} 
The following proposition shows that without further assumptions, a
non-trivial regret bound is impossible. Such results are common in the
RL literature, and motivate several structure assumptions, including
small diameter~\cite{jaksch2010near} and episodic
problems~\cite{dann2015sample,osband2016posterior}.

\insertprethmspacing
\begin{proposition}
  There exists a DOE problem where
  $\lim_{n\to\infty}
  \EEtt{\thetatrue\sim\pthetazero}[\lossn(\thetatrue, \policy) -
  \lossn(\thetatrue, \gopolicy)] = 1/2$.
\end{proposition}
\begin{proof}
  Consider a setting with uniform prior over two parameters
  $\theta_0,\theta_1$ with two actions $X_0,X_1$. Set
  $\lambda(\theta_0,D) = \one\{X_{1} \in D\}$ and similarly for
  $\lambda(\theta_1,\cdot)$. If $\thetatrue=\theta_0$, then
  $\gopolicy$ will repeatedly $X_0$ and incur cumulative (and final)
  loss $0$ and similarly when $\thetatrue=\theta_1$. On the other
  hand, the first decision for the decision maker must be the same for
  both choices of $\thetatrue$ and hence the regret is $1/2$.
\end{proof}
% We first need to
% acknowledge that achieving good regret without additional assumptions
% is impossible since the penalty is not observed.  For example, assume
% there exists an action $\badaction\in\Xcal$ such that for all data
% sequences $D$ which contain $\badaction$, we have maximum penalty
% $\penl(\thetatrue,D) = 1$.  While $\gopolicy$, which knows
% $\thetatrue$ and hence the penalty, will never choose that action, a
% policy which does not know $\thetatrue$ might do so, especially in the
% early exploration stages.

% Such pathological examples arise in infinite-horizon RL, and motivate
% recoverability or diameter conditions~\cite{jaksch2010near}, which we
% will also require. Another workaround from the RL literatue is to
% consider episodic settings. 

% This is similar to settings in infinite horizon reinforcement learning
% where a single bad action might us to a state from which we cannot recover.
% Most theoretical results for RL are in the episodic
% setting~\citep{dann2015sample,osband2016posterior}, where, even if we were to
% perform poorly in one episode, there is hope to do well in the long run since we start
% afresh at the next episode. 

% \toworkon{Why this is difficult without assumptions. Refer to RL literature.}
Motivated by this lower bound, we will study a variety of conditions
on the penalty function, under which a policy can achieve sub-linear
regret~\eqref{eqn:regretDefn}.  The first condition, inspired by some
of the above results in episodic RL, states that the penalty function
has episodic structure.
% That is, we can think of the 

% \insertprethmspacing
% \begin{condition}[Finite dependence on Actions]
% \label{cond:instantaneous}
% Let $K\in\NN_+$ and 
% let $\sigma:\NN \rightarrow 2^\NN$ be a deterministic function such that
% $t-K\leq s \leq t$ for all $s\in\sigma(t)$ and $|\sigma(t)| \leq K$.
% For a data sequence $\datat$, let $\datatt{t,\sigma(t)} = \{(\Xj,\YXj): j\in\sigma(t)\}$.
% Than, at any given time step, $\penl$ depends only on the actions and observations
% taken at the time steps in $\sigma(t)$;
% i.e. $\penl(\thetatrue,\datat) = \penl(\thetatrue,\datatt{t, \sigma(t)})$
% \end{condition}

\insertprethmspacing
\begin{condition}[Episodic Penalties]
% \label{cond:instantaneous}
\label{cond:instantaneous}
The infinite sequence can be divided into ``episodes'' of length $H$ where
episode $j$ consists of time steps $(j-1)H + 1$ to $jH$.
The penalty at a given time step depends only on the action and observation of the current
episode. That is, 
$\penl(\thetatrue,\datat) = \penl(\thetatrue,\{(\Xj, \YXj)\}_{j=t'}^t)$
and $t'$ is the start time of the current episode.
\end{condition}

% A simple example where Assumption~\ref{cond:instantaneous} holds is a moving average
% bandit where the reward at the current time step is the average of the last
% $K$ rewards.
\towillie{can you think of an example for this?}

A special case here is bandit optimization, which has $H=1$.  The next
condition under which we can achieve sub-linear regret is a notion of
recoverability. Intuitively, Condition~\ref{cond:recoverability}
states that it is possible to choose an action from a ``bad" data
sequence to improve, by a multiplicative factor of $\alpha$, in
comparison with choosing the best action from a ``good" data
sequence. This implies that even if we were unfortunate to have chosen
bad actions early on, there is opportunity to recover and eventually
start performing well.  Condition~\ref{cond:recoverability} is quite
similar to diameter/reachability conditions in
RL~\cite{jaksch2010near}, which assume that every state (in particular
a good state) is reachable from every other in a small number of
steps.

\insertprethmspacing
\begin{condition}[Recoverability]
\label{cond:recoverability}
There exists $\alpha<1$ such that for data sequences $D_1, D_2$ with
$\penl(\thetatrue, D_1) \leq \penl(\thetatrue, D_2) + \epsilon$,
we have the following for given $\thetatrue$.
The expectation
$\EEtt{\Yx}$ is over the the observation $\Yx$ at $x$.
% \vspace{-0.05in}
\[
\max_{x\in\Xcal} \EEtt{\Yx}[\penl(\thetatrue, D_1\concat (x,\Yx))]
\leq \max_{x\in\Xcal} \EEtt{\Yx}[\penl(\thetatrue, D_2\concat (x,\Yx))] +
\alpha\epsilon.
\]
\end{condition}
% \insertpostthmspacing



% Assume that we have two data sequences $D_1$ and $D_2$ where $D_1$ is worse than $D_2$
% by up to $\epsilon$.
% Condition~\ref{cond:recoverability} states that it is possible to choose a point with the
% ``bad'' dataset $D_1$, so as to improve on this slack by a factor $\alpha$ in comparison
% to the best point choosable with $D_2$.
% Intuitively, this states that even if we were unfortunate to have had bad observations
% and hence large penalty $\penl$, there is opportunity to
% recover and eventually start performing well.
% This condition is similar in spirit to results for infinite horizon RL which
% assume that the Markov decision process mixes fast enough so that one can recover from a
% bad state~\citep{jaksch2010near}.

The next condition assumes regularity on $\penl$ when collecting
data according to $\gopolicy$.
In particular, that $\gopolicy$ can make better decisions when it has more data.
We will show that when the myopic policy $\gopolicy$ which knows $\thetatrue$
can behave reasonably, so can posterior sampling $\pspolicy$.


\insertprethmspacing
\begin{condition}[More data is better]
  Let $D,D'\in\Dcal$ be data sequences such that $D \dssubset D'$.
  Let $H,H'$ be equal length ($|H| = |H'|$) data sequences
  collected by $\gopolicy$ when it starts from $D$ and $D'$ respectively.
%   Let $\Ytt{H}\in\Ycal^{|H|}$ be the observations when taking actions in $H$.
%     Define $\Ytt{H'}$ similarly.
  Then, for given $\thetatrue$, $\EE[\penl(\thetatrue, D'\concat H')] \leq
      \EE[\penl(\thetatrue, D\concat H)]$
  where the expectation is over the future sequences $H,H'$ collected
by $\gopolicy$.
% \label{cond:monotonicity}
\label{cond:moreisbetter}
\end{condition}
\akshay{Should we call this monotonicity or maybe diminishing returns?}


Note that the conditions~\ref{cond:recoverability} and~\ref{cond:moreisbetter}
are stated with respect to the true parameter $\thetatrue$;
i.e. that good actions \emph{can} be chosen so as to achieve certain conditions.
Hence, they are essentially conditions on the properties of the penalty function.
While a policy which knows $\thetatrue$, such as $\gopolicy$, which can compute the exact 
expected value of future penalties, can always correctly choose such actions,
this may not be the case for a policy such as $\pspolicy$ which does not know
$\thetatrue$.
 
To state our main theorem, we introduce the maximum information gain,
$\IGn$.
\begin{align*}
% \IRt &= \frac{\EEtmo[\penlt(\thetatrue,\datat) - \penlt(\thetatrue,\iodatat)]^2}{%
%  \Itmo(\thetatrue; (\Xt, \YXt)) }
% \numberthis\label{eqn:infratio}
%  \\
\IGn &= \max_{\datan\subset\Dcaln} \MI(\thetatrue; \datan).
\numberthis\label{eqn:mig}
\end{align*}
Here $\MI$ is the Shannon mutual information.
$\IGn$ measures the maximum information a set of $n$ action-observation pairs can
tell us about the true parameter $\thetatrue$.
The quantity was first introduced for Gaussian processes
by~\citet{srinivas10gpbandits}, and has been popularly
% used in regret bounds in various Bayesian adaptive data analysis settings such as
used to measure the statistical complexity of various Bayesian adaptive data analysis
settings such as Bayesian optimisation~\citep{srinivas10gpbandits},
active learning~\citep{ma2015active},
and level set estimation~\citep{gotovos2013active}.
Below, we list some examples of common models which demonstrate that
$\IGn$ is sublinear in $n$.

\insertprethmspacing
% \begin{example}[Bounds on the MIG for common models~\citep{srinivas10gpbandits}]
\begin{example}Bounds on the maximum information gain for common models~\cite{srinivas10gpbandits}.
\vspace{-0.02in}
\begin{enumerate}[leftmargin=0.3in]
\setlength\itemsep{-0.02in}
\item \textbf{Finite sets:}
If $\Theta$ is a finite set, $\IGn \leq \log(|\Theta|)$ for all $n$.
\item \textbf{Linear models:}
Let $\Xcal\subset\RR^d$, $\theta\in\RR^d$,
 and $\Yx|x,\theta \sim\Ncal(\theta^\top x, \eta^2)$.
For a multi-variate Gaussian prior on $\thetatrue$, $\IGn\in\bigO(d\log(n))$.
\item \textbf{Gaussian process:}
Let $\Xcal\subset\RR^d$.
Assume a Gaussian process prior
$\thetatrue\sim\GP(\mu,\kernel)$,
and Gaussian observations $\Yx|x,\theta \sim\Ncal(\theta(x), \eta^2)$.
Here $\mu:\Xcal\rightarrow\RR$ is the prior mean of the GP and
$\kernel:\Xcal^2\rightarrow\RR$ is the covariance kernel.
When $\kernel$ is an RBF kernel, $\IGn\in\bigO(\log(n)^{d+1})$.
When $\kernel$ is a mat\'ern kernel, $\IGn\in\bigO(n^p\log(n))$ for some $p<1$.
\end{enumerate}
% \vspace{-0.10in}
% \begin{proof}
% For finite $\Theta$, we have $\MI(\thetatrue, \datan) = \Ent(\thetatrue) -
% \Ent(\thetatrue|\datan) \leq \Ent(\thetatrue) \leq \log(|\Theta|)$,
% where $\Ent$ is the shannon Entropy.
% The last two results are taken from~\citet{srinivas10gpbandits}.
% \end{proof}
\end{example}
\insertpostthmspacing

% In general, one expects the regret in an interactive model to depend on the complexity
% of the model and 
% While the MIG is not known
% The MIG provides us a way to abstract out the statistical complexity of a model.
We now state our main theorem for finite action spaces $\Xcal$
under any one of the above conditions.

\insertprethmspacing
\begin{theorem}
\label{thm:finiteactions} 
Assume \textbf{any one} of conditions~\ref{cond:instantaneous}-\ref{cond:moreisbetter}
hold.
Let $B=H$ under condition~\ref{cond:instantaneous},
$B=1/(1-\alpha)$ under condition~\ref{cond:recoverability},
% $B=1$ under condition~\ref{cond:monotonicity},
and $B=2$ under condition~\ref{cond:moreisbetter}.
Then if $\Xcal$ is finite,
\[
\EE[\lossn(\thetatrue,\pspolicy) - \lossn(\thetatrue, \gopolicy)]
\leq B\sqrt{\frac{1}{2}n|\Xcal|\IGn}
\]
\end{theorem}
\akshay{No bound on $\penl(\thetatrue,D_n)$ here?}

Theorem~\ref{thm:finiteactions} establishes a sublinear regret bound for $\pspolicy$
against $\gopolicy$.
The $|\Xcal|$ term captures the complexity of our action space and
$\IGn$ captures the complexity of the prior on $\thetatrue$.
The $\sqrt{n}$ dependence is similar to other known results for
Thompson sampling in bandit and reinforcement learning
settings~\citep{kaufmann2012thompson,osband2016posterior,russo2016thompson}.
% In addition, the $\IGn$ term captures the statistical di

Next, we wish to compare $\pspolicy$ against the globally optimal
adaptive policy $\uopolicy$. 
% , and in particular,
% study conditions under which it can perform favourably.
% For what follows, we will find it convenient to define $\reward = 1-\penl$, which
% can be interpreted as a reward for collecting a data sequence.
To do so, we introduce the notion of adaptive submodularity and
monotonicity~\cite{golovin2011adaptive}, under which it is known that
$\gopolicy$ closely approximate $\uopolicy$.  Monotonicity states that
adding more data reduces the penalty in expectation, while adaptive
submodularity formalizes a notion of diminishing returns; the expected
benefit in carrying out a particular action is larger when we have
less data.

% A line of work~\citep{golovin2011adaptive,gabillon2013adaptive} has shown that,
% in settings where the penalty is known or observed,
% greedy strategies can perform competitively with the globally
% optimal policy, if the reward is monotone and
% satisfies a diminishing returns property called adaptive submodularity.
% We demonstrate that under similar assumptions on the penalty function for given
% $\thetatrue$, a similar guarantee can be obtained for posterior sampling even
% though the penalty is now observed.
% We state this condition formally below.


\insertprethmspacing
\begin{condition}(Monotonicity and Adaptive Submodularity)
\label{cond:submod}
Let $D, D'$ be such that $D\dssubset D'$.
Then, the penalty $\penl$ is monotone, i.e 
for all $x\in\Xcal$, 
$\EE_{\Yx}[\penl(\thetatrue, D\concat\{(x, \Yx)\})]
\leq  \penl(\thetatrue, D)$.
The penalty $\penl$ is adaptive submodular if it satisfies
$\EEobs[\penl(\thetatrue, D\concat\{(x,\Yx)\})] - \penl(\thetatrue,D)
\geq 
\EEobs[\penl(\thetatrue, D'\concat\{(x,\Yx)\})] - \penl(\thetatrue,D)$.
\end{condition}

% Both conditions above are natural in adaptive data collection settings and
% have been used in the adaptive submodularity literature~\citep{gabillon2013adaptive,%
% gotovos2013active}.

% For what follows, we will find it useful to define $\reward = 1-\penl$, which
% can now be interpreted as a reward for collecting a data sequence.
% Recall that by the definition of $\uopolicy$, the data sequence $\uodatan$
% maximises
% $\EE[\reward(\thetatrue, \datan)]$ over all adaptive data choices $\datan$.
We have the following result for $\pspolicy$ under the above conditions.
% The result below shows


\insertprethmspacing
\begin{theorem}
\label{thm:submodthm}
Assume that $\penl$ satisfies condition~\ref{cond:submod} and one of
conditions~\ref{cond:instantaneous}-\ref{cond:moreisbetter}.
Let $\mu = 1 - \penl$.
Let $\datan, \uodatan$ be the data sequences collected by $\pspolicy$ and
$\uopolicy$ respectively in $n$ experiments.
Let $B$ be as defined in Theorem~\ref{thm:finiteactions}.
Then, for all $\gamma < 1$, we have the following two equivalent statements.
\begin{align*}
\EE[\penl(\thetatrue, \datan)]
&\;\leq\; \EE[\penl(\thetatrue,\uodatagn)] +
\gamma(1 -  \EE[\penl(\thetatrue,\uodatagn)]) + 
B \sqrt{\frac{|\Xcal|\IGn}{2n}}. \\
\EE[\reward(\thetatrue, \datan)]
&\;\geq\; (1 - \gamma) \EE[\reward(\thetatrue, \uodatagn)] -B \sqrt{\frac{|\Xcal|\IGn}{2n}}.
\end{align*}
\end{theorem}

% When $\reward = 1-\penl$ is viewed as a reward,
In terms of rewards, the theorem states that $\pspolicy$ in $n$ steps
is guaranteed to perform up to a $1-\gamma$ factor as well as the
globally optimal policy executed for $\gamma n \le n$ steps, up at an
additive $\sqrt{\IGn/n}$ term. The result captures both approximation
and estimation errors, in the sense that we are using a myopic policy
to approximate a globally optimal one, and we are learning a good
myopic policy from data. In comparison, prior works on adaptive
submodular optimization focus on approximation errors and typically
achieve $1-1/e$ approximation ratios against the $n$ steps of
$\uopolicy$. Our bound is quantitatively worse, but focusing on a much
more difficult task, and we view the results as complementary.
% The latter term vanishes as $n\rightarrow\infty$ so, asymptotically $\pspolicy$ achieves
% this constant factor.
% This result is analogous to well known results in submodular \emph{maximisation}
% where greedy policies are known to achieve up to a constant factor of the 
% global maximum.
% However, while adaptive submodular maximisation is known to achieve a
% $1-1/e$ approximation to the global optimum executed for $n$ steps,
% $\pspolicy$ can only achieve this for $\gamma n$ steps, and moreover,
% the constant factor decreases with $\gamma$.
% Hence, the result in Theorem~\ref{thm:submodthm} is weaker than submodular maximisation
% in two aspects.
% We believe that this is primarily due to the fact that the rewards are not known or
% observed which makes our settings considerably more challenging
% than classical submodular maximisation.
We finally note that an analogous bound holds against $\gopolicy$, since it is necessarily worse that $\uopolicy$.
%  statement akin to Theorem~\ref{thm:submodthm} can also
% be stated with respect to the myopic policy $\gopolicy$ since it is necessarily
% worse than $\uopolicy$.


\akshay{I suggest we state one of these formally. Probably the
  infinite action case is most relevant.}  Finally, we mention that
the above results can be generalised to very large or infinite action
spaces, using known techniques~\citep{russo2016thompson,bubeck2011x};
this is tangential to the goal of this paper.
Algorithm~\ref{alg:bdoe} can be applied as is in either synchronously
or asychronously parallel settings with $m$ workers.  By following
analysis techniques for parallelised Thompson sampling for Bayesian
optimisation~\citep{kandasamy2018parallel}, we believe that one can
obtain results similar to Theorems~\ref{thm:finiteactions}
and~\ref{thm:submodthm} with mild dependence on $m$.


